Efficient Loop Conditions for Bounded Model Checking Hyperproperties

Bounded model checking (BMC) is an effective technique for hunting bugs by incrementally exploring the state space of a system. To reason about infinite traces through a finite structure and to ultimately obtain completeness, BMC incorporates loop conditions that revisit previously observed states. This paper focuses on developing loop conditions for BMC of HyperLTL- a temporal logic for hyperproperties that allows expressing important policies for security and consistency in concurrent systems, etc. Loop conditions for HyperLTL are more complicated than for LTL, as different traces may loop inconsistently in unrelated moments. Existing BMC approaches for HyperLTL only considered linear unrollings without any looping capability, which precludes both finding small infinite traces and obtaining a complete technique. We investigate loop conditions for HyperLTL BMC, where the HyperLTL formula can contain up to one quantifier alternation. We first present a general complete automata-based technique which is based on bounds of maximum unrollings. Then, we introduce alternative simulation-based algorithms that allow exploiting short loops effectively, generating SAT queries whose satisfiability guarantees the outcome of the original model checking problem. We also report empirical evaluation of the prototype implementation of our BMC techniques using Z3py.

==> cases.tex <==
%\pagebreak
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Implementation and Experiments}

Encode SAT query for each question manually using Z3 API in python.

%\subsection{Simple Examples}
%
%All small examples including $\forall\exists \G \varphi$ and $\exists\forall \G \varphi$ from the previous sections.
%\begin{figure}[h!]
%	\begin{minipage}{.45\textwidth}
%		\scalebox{0.6}{
%			\begin{tikzpicture}[-,>=stealth,shorten >=.5pt,auto,node distance=2cm, semithick, initial text={}]
%				\node[initial, state] [text width=1em, text centered, minimum  height=2.0em](0) at (0,0) {\hspace*{-0.8mm}$\{ \}$};
%				\node[above left = 0.005 cm and -0.1 cm of 0](label){\Large$s_1$};
%				%
%				\node[state][text width=1em, text centered, minimum 
%				height=2.5em] (1) at (2,0) {\hspace*{-0.8mm}$\{ \}$};
%				\node [above left = 0.005 cm and -0.1 cm of 1](label){\Large$s_{2}$};
%				%
%				\node[state][text width=1em, text centered, minimum 
%				height=2.5em] (2) at (4,1){\hspace*{-0.8mm}$\{a\}$};
%				\node [above left = 0.005 cm and -0.1 cm of 2](label){\Large$s_{3}$};
%				%
%				\node[state][text width=1em, text centered, minimum 
%				height=2.5em] (3) at (4,-1){\hspace*{-0.8mm}$\{ \}$};
%				\node [above left = 0.005 cm and -0.1 cm of 3](label){\Large$s_{4}$};
%				%
%				\draw[->]  
%				(0)	edge  node (01 label) {} (1)
%				(1) edge node (12 label) {} (2)
%				(1) edge node (03 label) {} (3)
%				(2) edge [bend right] node (03 label) {} (0)
%				(3) edge [bend left] node (03 label) {} (0);
%			\end{tikzpicture}
%		}
%		\caption {$M_A$}
%		\label{fig:kripke1}
%	\end{minipage}
%	%
%	\begin{minipage}{.45\textwidth}
%		\scalebox{0.6}{
%			\begin{tikzpicture}[-,>=stealth,shorten >=.5pt,auto,node distance=2cm, semithick, initial text={}]
%				\node[initial, state] [text width=1em, text centered, minimum  height=2.0em](0) at (0,0) {\hspace*{-0.8mm}$\{ \}$};
%				\node[above left = 0.005 cm and -0.1 cm of 0](label){\Large$q_1$};
%				%
%				\node[state][text width=1em, text centered, minimum 
%				height=2.5em] (1) at (2,1) {\hspace*{-0.8mm}$\{ \}$};
%				\node [above left = 0.005 cm and -0.1 cm of 1](label){\Large$q_{2}$};
%				%
%				\node[state][text width=1em, text centered, minimum 
%				height=2.5em] (2) at (2,-1){\hspace*{-0.8mm}$\{ \}$};
%				\node [above left = 0.005 cm and -0.1 cm of 2](label){\Large$q_{3}$};
%				%
%				\node[state][text width=1em, text centered, minimum 
%				height=2.5em] (3) at (4,1){\hspace*{-0.8mm}$\{a\}$};
%				\node [above left = 0.005 cm and -0.1 cm of 3](label){\Large$q_{4}$};
%				%
%				\node[state][text width=1em, text centered, minimum 
%				height=2.5em] (4) at (4,-1){\hspace*{-0.8mm}$\{ \}$};
%				\node [above left = 0.005 cm and -0.1 cm of 4](label){\Large$q_{5}$};
%				
%				%
%				\draw[->]  
%				(0)	edge  node (01 label) {} (1)
%				(0)	edge  node (01 label) {} (2)
%				(1) edge node (12 label) {} (3)
%				(2) edge node (03 label) {} (4)
%				(3) edge [bend right=85] node (03 label) {} (0)
%				(4) edge [bend left=60] node (03 label) {} (0);
%			\end{tikzpicture}
%		}
%		\caption {$M_B$}
%		\label{fig:kripke2}
%	\end{minipage}
%\end{figure}


\subsection{Matrix Multiplication (Certificate Translation)}
It is often the case that reasoning about source programs dies not provide guarantees about the desirable behavior of the executable code. 
In [Barthe'09], {\em certificate translation} can can take inputs of high-level programs (source) with a defined specification, and compute a set of verification conditions for the low level implementation (target). 
Here we argue that with our simulation technique can directly proof the same thing, that is, specification preserved from the source to target. 


Consider a program that compute the multiplication of the following $2 \times 2$ matrix:
$$
\begin{pmatrix}
	a & b\\
	c & d
\end{pmatrix}
$$
Consider a C-style implementation, where a matrix is represented by an uni-dimensional array, that computes the multiplication of a matrix, is as follows:

\begin{minipage}{.93\textwidth}
\begin{algorithm}[H]
	\setcounter{AlgoLine}{0}
	$i := 0;$ \\
	\While{i < m}
	{
		$j := 0;$ \\
		\While{j < p}
		{
			$k := 0;$ \\
			\code{c[ i $\ast$  p + j ]} := 0; \\
			\While{k < n}
			{
				\code{c[ i $\ast$  p + j ]} := \code{c[ i $\ast$  p + j ]} + \code{a[ i $\ast$  n + k ]} $\ast$ \code{b[k $\ast$  p + j ]}; \\
				$k := k+1;$
			}
		$j := j+1;$
		}
	$i := i+1;$
	}
	\Return{0}
	\caption{Source Program of Matrix Multiplication.}
\end{algorithm}
\end{minipage}

The procedure specification in [Barthe'09] are triples of $\langle Pre, annot, Post \rangle$, where $Pre$, and $Post$ are assertions and $annot$ is a partial function from labels to assertions. 
In our framework, all three elements can be expressed as {\em hyperproperties}. That is, instead of translating the specification, we make sure that for all source executions, there exists a target executions, which preserves that the specification fulfilled by the source will also be fulfilled by the target. 

\includegraphics[scale=.25]{figs/spec}
%$$Pre  \dot{=} (0 < m) \land (0 < n) \land (0 < p) $$
%$$\ldots$$


A matrix multiplication program that is translated from high-level code (C)  to low-level code (RTL-- Register Transfer Level). Instead of translating the certificate, we find simulation.

\begin{minipage}{.93\textwidth}
	\begin{algorithm}[H]
		{\includegraphics[scale=.2]{figs/matrix_exists}}
		\caption{Target Program of Matrix Multiplication.}
	\end{algorithm}
\end{minipage}


To check if a translation is valid, we check: 
$$ \varphi = \forall \pi. \exists \pi'. \G\ (p_\pi \leftrightarrow p_{\pi'})$$

%\fbox{\includegraphics[scale=.3]{matrix_forall}}
%\fbox{\includegraphics[scale=.3]{matrix_prop}}
%\fbox{\includegraphics[scale=.2]{matrix_exists}}

\newcommand{\sender}{\texttt{sender}}
\newcommand{\receiver}{\texttt{receiver}}
\newcommand{\send}{\textit{send}}
\newcommand{\receive}{\textit{receive}}
\newcommand{\wait}{\textit{wait}}
\subsection{Alternating-Bit Protocol (Scenario-based Synthesis)}

Synthesize a implementation from a set of scenarios augmented with a set of safety properties, provided the given scenarios adequately cover all the states of the desired implementation. Instead of independently check the synthesized protocol (HVC'14), instead, we find a simulation between the scenarios and the synthesized outcome. 


%\fbox{\includegraphics[scale=.2]{abp_forall}}

%\fbox{\includegraphics[scale=.2]{abp_exists}}

The protocol has two parties: \sender\ and \receiver, where they can take three different actions: \send, \receive, and \wait. Each action is also specified by which message is currently transmitted, which is either a {\em packet} or {\em acknowledgment.} (denoted as $p_i$ and $a_i$, where $i$ is simply the index to distinguish different messages). 

%\hspace{-5mm}
\begin{minipage}{.55\textwidth}
	\begin{algorithm}[H]
		\setcounter{AlgoLine}{0}
		\While{true}
		{
		$\sender.\send(p_0)$ \\
		$\receiver.\receive(p_0)$ \\
		$\receiver.\send(a_0)$ \\
		$\sender.\receive(a_0)$ \\
		$\sender.\send(p_1)$ \\
		$\receiver.\receive(p_1)$ \\
		$\receiver.\send(a_1)$ \\
		$\sender.\receive(a_1)$ \\
		}
		\caption{ABP-\emph{no loss}.}
	\end{algorithm}
\end{minipage}
%

%
\begin{minipage}{.55\textwidth}
	\begin{algorithm}[H]
		\setcounter{AlgoLine}{0}
		\While{true}
		{
			$\sender.\send(p_0)$ \\
			$\receiver.\receive(p_0)$ \\
			$\receiver.\send(a_0)$ \\
			$\sender.\receive(a_0)$ \\
			$\sender.\send(p_1)$ \\
			\If{packet-loss}{ go back to 6.}
			$\receiver.\receive(p_1)$ \\
			$\receiver.\send(a_1)$ \\
			$\sender.\receive(a_1)$ \\
		}
		\caption{ABP-\emph{packet loss}.}
	\end{algorithm}
\end{minipage}
%

%
\begin{minipage}{.55\textwidth}
	\begin{algorithm}[H]
		\setcounter{AlgoLine}{0}
		\While{true}
		{
			$\sender.\send(p_0)$ \\
			$\receiver.\receive(p_0)$ \\
			$\receiver.\send(a_0)$ \\
			$\sender.\receive(a_0)$ \\
			$\sender.\send(p_1)$ \\
			$\receiver.\receive(p_1)$ \\
			$\receiver.\send(a_1)$ \\
			\If{ack-loss}{ go back to 6.}
			$\sender.\receive(a_1)$ \\
		}
		\caption{ABP-\emph{ack loss}.}
	\end{algorithm}
\end{minipage}

The synthesized protocol should not only have complete functionality but also {\em include all scenarios}. That is, the for all traces appear in any of the scenarios, there must be a corresponding trace exists in the synthesized protocol. 

In this example, we consider (1) a manually built ABP, and (2) a synthesized ABP, from [HVC'14] which the models are as follows:

\includegraphics[scale=.3]{figs/abp_exists} 

Finally, to verify whether a synthesis is correct, we check: 

Given two programs -- scenarios (\msmall) and synthesized protocol (\mbig) 
$$ \varphi = \forall \pi. \exists \pi'. \G\ (p_\pi \leftrightarrow p_{\pi'})$$
example: {\em HVC'14}, APB Protocols
%  



\subsection{Secure Compilation}

Compile from source program to target program that preserves the security property. 
The below target program violates confidentiality:

The source and target programs are identical as the CCS'22 paper.

%Given two programs -- target (\mbig)and source (\msmall)
%$$ \varphi = \forall \pi. \exists \pi'. \G\ (\violation_\pi \rightarrow \violation_{\pi'})$$
%examples: {\em witnessing\_secure\_compilation}

%\vspace{3mm}
%\fbox{\includegraphics[scale=.3]{sc}}
%\vspace{3mm}

%{\question Q: Can this be captured by $\forall \exists$?}

%\bibliographystyle{plainurl}
%\bibliography{bibliography}


\subsection{(New) Software Architectural Specification}
 
 Software architecture (SA) has emerged as an autonomous discipline. Through suitable abstractions, it provides the means to make large applications manageable.
 Recently, various approaches have been proposed on testing driven by the architectural specification. Our goal is to provide a test manager with a systematic method to extract suitable test classes for the higher levels of testing and to refine them into concrete tests at the code level. Essentially: 
 $$
 \text{Software architecture (SA) in LTSs} \rightarrow \text{Abstract LTSs} \rightarrow \text{code-level test}
 $$
 We use the example from [IEEE'04]. The Teleservice and Remote Medical Care System (TRMCS) [32] is a system that provides monitoring and assistance to disabled or elderly people; containing: User, Router, Server, Timer.  
 
 Step 1: Model.

 \includegraphics[scale=.3]{figs/1}
 
 Step 2: Abstraction.
 
  \includegraphics[scale=.3]{figs/2}
 
 
 Step 3: code-level test.
 
  \includegraphics[scale=.3]{figs/3}
  
 Check traceability. Traceability concerns “relating the abstract values of the specification to the concrete values of the implementation”
 
 For step 3,  we can replaced as a simulation search using our approach. Instead of checking the behavior of each component by the Finite State Process (FSP) generated by LTS, we can simply find the simulation and check conformance between the abstraction and the implementation.
 
  
 































==> completeness.tex <==
%\pagebreak
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Completeness and Applications}
%%%%%%%%%%%% TABLE %%%%%%%%%%%%

{\bf Contributions:} \\
\aesim, \easim, and we use {prophecy variables for non-deterministic models}.\\

\noindent{\bf Goal:}\\
If a simulation exists, the following implications hold:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
	\renewcommand{\arraystretch}{1.2}
	\centering % used for centering table
	\scalebox{1}{
		\input{table_complete}
	}
	\vspace{3mm}
%	\caption{Cases of \hltl verification, where $\varphi$ is a {\em hyperproperty} that can be expressed with {\em local relational state predicate}. 
%	If simulation (\aesim, \easim) exists, then the two programs agree on $\varphi$, else, a {\em counterexample} can be derived by BMC bug hunting.
%	For \aesim, a set of {\em prophecy variables} can be manually added to different states for correctness guarantee .}
	\label{tab:results}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
	\input{table_exp}
\end{table}

\noindent{\bf Applications:}

\newcommand{\violation}{\text{violation}}
\begin{itemize}
	%
	\item Verification of secure compiler optimization: \\
	Given two programs -- target (\mbig)and source (\msmall)
	$$ \varphi = \forall \pi. \exists \pi'. \G\ (\violation_\pi \rightarrow \violation_{\pi'})$$
	examples: {\em witnessing\_secure\_compilation}
	%
	\item Verification of scenario-based synthesis: \\
	Given two programs -- scenarios (\msmall) and synthesized protocol (\mbig) 
	$$ \varphi = \forall \pi. \exists \pi'. \G\ (p_\pi \leftrightarrow p_{\pi'})$$
	example: {\em HVC'14}, APB Protocols
	%
	\item Verification of model translations(semantic/behavioral conformance).\\
	$$ \varphi = \forall \pi. \exists \pi'. \G\ (p_\pi \leftrightarrow p_{\pi'})$$
	example: {\em Barthe'09}, Matrix Multiplication
	%
	\item Verification of relational property without program composition.
	\begin{itemize}
		\item translation validation 
		\item predicate abstraction
	\end{itemize}
	\item Verification of equivalence for database-driven applications.
\end{itemize}

%{\color{red} Our simulation definitions v.s. bi-simulation?}

%\pagebreak
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Implementation and Experiments}
%
%Encode SAT query for each question manually using Z3 API in python.
%
%\subsection{Simple Examples}
%
%All small examples including $\forall\exists \G \varphi$ and $\exists\forall \G \varphi$.
%
%{\question Q: arbitrary temporal formulas?}\\
%{\question Q: automated tool?}\\
%
%
%\subsection{Matrix Multiplication (Certificate Translation)}
%
%A matrix multiplication program that is translated from high-level code (C)  to low-level code (RTL). Instead of translating the certificate, we find simulation.
%
%\fbox{\includegraphics[scale=.3]{matrix_forall}}
%
%\fbox{\includegraphics[scale=.3]{matrix_prop}}
%
%\fbox{\includegraphics[scale=.2]{matrix_exists}}
%
%\subsection{Alternating-Bit Protocol (Scenario-based Synthesis)}
%
%Synthesize a implementation from a set of scenarios augmented with a set of safety properties, provided the given scenarios adequately cover all the states of the desired implementation.
%
%
%\fbox{\includegraphics[scale=.2]{abp_forall}}
%
%\fbox{\includegraphics[scale=.2]{abp_exists}}
%
%
%\subsection{Secure Compilation}
%
%Compile from source program to target program that preserves the security property. 
%The below target program violates confidentiality:
%
%\vspace{3mm}
%\fbox{\includegraphics[scale=.3]{sc}}
%\vspace{3mm}
%
%{\question Q: Can this be captured by $\forall \exists$?}

%\bibliographystyle{plainurl}
%\bibliography{bibliography}
%\end{document}
































==> exp_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\scalebox{.9}{
\begin{tabular}{| L{.53cm}|M{.68cm}|M{5.6cm}|P{.2cm}|M{.4cm}|M{.35cm}  |M{.35cm}|M{.35cm} | M{1cm} |} 
%	\hline
% Header
	
	\\ \hline	
\end{tabular}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%
%
%
%%%% 
%\begin{table*}[h!]
%\renewcommand{\arraystretch}{1.3}	
%\newcommand{\graphscale}{.85}
%\newcommand{\textscale}{\scriptsize}
%\centering % used for centering table
%\scalebox{1.4}{
%\begin{tabular}{ ||M{2.3cm} | M{2.3cm} | M{1cm} | M{1cm} | M{1cm} ||} 
%	\hline
%	{\bf Properties} & {\bf Cases}  & {\bf LoC} & {\bf \# States} &{\bf Synth[s]}\\
%	\hline \hline
%	NI & login.html  & & & \\ \hline			
%	NI & implicit\_flow1.js  & & & \\ \hline
%	NI & implicit\_flow2.js  & & & \\ \hline
%	NI & sunspider-crypto-md5 & & & \\ \hline
%	Ninf & login.html  & & & \\ \hline
%	NI-Declassification &   & & & \\ \hline
%	Ninf-Declassification & gps.js  & & & \\ \hline
%	Code Injection & & & & \\ \hline
%	Buffer Vulnerability & & & & \\ \hline
%	Device Fingerprinting & & & & \\ \hline
%	History Sniffing & & & & \\ \hline
%\end{tabular}

==> fig_abp.tex <==
\begin{subfigure}{.31\linewidth}
	\centering
	%		\includegraphics{image1}
	\boxed{placeholder}
	\caption{Packet loss.}
	\label{fig:abp1}
\end{subfigure}%
\begin{subfigure}{.31\linewidth}
	\centering
	%		\includegraphics{image2}
	\boxed{placeholder}
	\caption{Ack loss.}
	\label{fig:abp2}
\end{subfigure}
\begin{subfigure}{.31\linewidth}
	\centering
	%		\includegraphics{image3}
	\boxed{placeholder}
	\caption{Timeout.}
	\label{fig:abp3}
\end{subfigure}


%\begin{figure}[tbh!]
%\begin{minipage}{.3\textwidth}
%	\begin{algorithm}[H]
	%		\setcounter{AlgoLine}{0}
	%		\While{true}
	%		{
		%			$\sender.\send(p_0)$ \\
		%			$\receiver.\receive(p_0)$ \\
		%			$\receiver.\send(a_0)$ \\
		%			$\sender.\receive(a_0)$ \\
		%			$\sender.\send(p_1)$ \\
		%			$\receiver.\receive(p_1)$ \\
		%			$\receiver.\send(a_1)$ \\
		%			$\sender.\receive(a_1)$ \\
		%		}
	%		\caption{ABP-\emph{no loss}.}
	%	\end{algorithm}
%\end{minipage}
%%
%%
%\begin{minipage}{.3\textwidth}
%	\begin{algorithm}[H]
	%		\setcounter{AlgoLine}{0}
	%		\While{true}
	%		{
		%			$\sender.\send(p_0)$ \\
		%			$\receiver.\receive(p_0)$ \\
		%			$\receiver.\send(a_0)$ \\
		%			$\sender.\receive(a_0)$ \\
		%			$\sender.\send(p_1)$ \\
		%			\If{packet-loss}{ go back to 6.}
		%			$\receiver.\receive(p_1)$ \\
		%			$\receiver.\send(a_1)$ \\
		%			$\sender.\receive(a_1)$ \\
		%		}
	%		\caption{ABP-\emph{packet loss}.}
	%	\end{algorithm}
%\end{minipage}
%%
%%
%\begin{minipage}{.3\textwidth}
%	\begin{algorithm}[H]
	%		\setcounter{AlgoLine}{0}
	%		\While{true}
	%		{
		%			$\sender.\send(p_0)$ \\
		%			$\receiver.\receive(p_0)$ \\
		%			$\receiver.\send(a_0)$ \\
		%			$\sender.\receive(a_0)$ \\
		%			$\sender.\send(p_1)$ \\
		%			$\receiver.\receive(p_1)$ \\
		%			$\receiver.\send(a_1)$ \\
		%			\If{ack-loss}{ go back to 6.}
		%			$\sender.\receive(a_1)$ \\
		%		}
	%		\caption{ABP-\emph{ack loss}.}
	%	\end{algorithm}
%\end{minipage}
%\end{figure}
%
%\includegraphics[scale=.3]{figs/abp_exists} 

==> fig_matrix.tex <==
\begin{subfigure}{.5\linewidth}
	\centering
	%		\includegraphics{image1}
	\boxed{placeholder}
	\caption{Matrix-Mult Source}
	\label{fig:matrix1}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
	\centering
	%		\includegraphics{image2}
	\boxed{placeholder}
	\caption{Matrix-Mult Target}
	\label{fig:matrix2}
\end{subfigure}\\[1ex]
\begin{subfigure}{\linewidth}
	\centering
	%		\includegraphics{image3}
	\boxed{placeholder}
	\caption{Matrix-Mult Specifications}
	\label{fig:matrix3}
\end{subfigure}



%$$
%\begin{pmatrix}
%	a & b\\
%	c & d
%\end{pmatrix}
%$$

%
%\begin{minipage}{.93\textwidth}
%	\begin{algorithm}[H]
	%		\setcounter{AlgoLine}{0}
	%		$i := 0;$ \\
	%		\While{i < m}
	%		{
		%			$j := 0;$ \\
		%			\While{j < p}
		%			{
			%				$k := 0;$ \\
			%				\code{c[ i $\ast$  p + j ]} := 0; \\
			%				\While{k < n}
			%				{
				%					\code{c[ i $\ast$  p + j ]} := \code{c[ i $\ast$  p + j ]} + \code{a[ i $\ast$  n + k ]} $\ast$ \code{b[k $\ast$  p + j ]}; \\
				%					$k := k+1;$
				%				}
			%				$j := j+1;$
			%			}
		%			$i := i+1;$
		%		}
	%		\Return{0}
	%		\caption{Source Program of Matrix Multiplication.}
	%	\end{algorithm}
%\end{minipage}

%\includegraphics[scale=.25]{figs/spec}

%\begin{minipage}{.93\textwidth}
%	\begin{algorithm}[H]
	%		{\includegraphics[scale=.2]{figs/matrix_exists}}
	%		\caption{Target Program of Matrix Multiplication.}
	%	\end{algorithm}
%\end{minipage}
%



==> figs/ipe/latex/definitions.tex <==
\newcommand{\Terms}{\mathcal{T}}


%
\newcommand{\Str}{\mathcal{S}} \newcommand{\StrDesc}{\Rightarrow}
\newcommand{\StrReaches}{\StrDesc^*} \newcommand{\Desc}{\mapsto}
\newcommand{\DirDesc}{\rightarrow}
%
\newcommand{\RecDesc}{\twoheadrightarrow}
\newcommand{\AnyDesc}{\rightsquigarrow}
\newcommand{\AlphaDesc}{\dasharrow}
\newcommand{\ALPHADesc}[1]{\stackrel{#1}\dasharrow}
\newcommand{\Reaches}{\AnyDesc^*}
\newcommand{\Class}[1]{\ensuremath{[#1]}}
\newcommand{\EqSite}[2]{#1\equiv_{\Reactors}#2}
\newcommand{\LiveP}{\textsc{Live-P}\xspace}
\newcommand{\SchemaP}{\textsc{Schema-P}\xspace}
\newcommand{\BadP}{\textsc{Bad-P}\xspace} \newcommand{\INVname}{\phi}
\newcommand{\INV}{\ensuremath{\INVname}\xspace}
%
\newcommand{\INVnext}[2]{\ensuremath{\INVname_{#1}^{({#2})}}}
\newcommand{\INVclause}[1]{\ensuremath{\INVname[#1]}}
\newcommand{\INVnextclause}[3]{\ensuremath{\INVname_{#1}^{({#2})}[#3]}}
\newcommand{\React}[1]{\text{react}(#1)} \newcommand{\bisim}{\approx}
\newcommand{\Await}{\mathbf{await}} \newcommand{\When}{\mathbf{when}}
\newcommand{\Do}{\mathbf{do}} \newcommand{\Dec}{\texttt{--}}
\newcommand{\Inc}{\texttt{++}} \newcommand{\Width}{6em}
\newcommand{\Type}[1]{\hspace{-0.2em}:\hspace{-0.2em}#1} %
\newcommand{\LHeight}{\textit{lh}} \newcommand{\Height}{\textit{h}}
\newcommand{\owise}{\text{otherwise}}
\newcommand{\EmptyP}{\textsc{Empty-P}\xspace}
\newcommand{\AdequateP}{\textsc{Adequate-P}\xspace}
\newcommand{\BasicP}{\textsc{Basic-P}\xspace}
\newcommand{\BasicPRec}{\textsc{BasicRec-P}\xspace}
\newcommand{\EfficientP}{\textsc{Efficient-P}\xspace}
\newcommand{\kEfficientP}{\ensuremath{k}\textsc{-Efficient-P}\xspace}
\newcommand{\jEfficientP}{\ensuremath{j}\textsc{-Efficient-P}\xspace}
\newcommand{\Proc}{\mathcal{P}}
\newcommand{\WaitOnConnection}{\emph{WaitOnConnection}\xspace}
\newcommand{\WaitOnReactor}{\emph{WaitOnReactor}\xspace}
\newcommand{\process}{task\xspace}
\newcommand{\emprocess}{\emph{task}\xspace}
\newcommand{\processes}{tasks\xspace}
\newcommand{\emprocesses}{\emph{tasks}\xspace}
\newcommand{\subprocess}{sub-task\xspace}
\newcommand{\emsubprocess}{\emph{sub-task}\xspace}
\newcommand{\subprocesses}{sub-tasks\xspace}
\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\AllocName}{\textit{alloc}}
\newcommand{\Alloc}[1]{\textit{alloc\textup{(}[#1]\textup{)}}}
\newcommand{\AllocBigger}[1]{\textit{alloc.bigger\textup{(}#1\textup{)}}}
\newcommand{\AllocInc}[1]{\textit{alloc.inc\textup{(}#1\textup{)}}}
\newcommand{\AllocDec}[1]{\textit{alloc.dec\textup{(}#1\textup{)}}}
\newcommand{\p}[1]{\ensuremath{a[#1]}}
%
\newcommand{\Pplus}[1]{\ensuremath{A[#1]}}
\newcommand{\pnext}[2]{\ensuremath{a'_{#1}[#2]}}
\newcommand{\Pplusnext}[2]{\ensuremath{A'_{#1}[#2]}} %
\newcommand{\En}[2]{\mathit{En}_{#1}(#2)} %
\newcommand{\In}[2]{\mathit{In}_{#1}(#2)} %
\newcommand{\Out}[2]{\mathit{Out}_{#1}(#2)} %
\newcommand{\Pres}[1]{\mathit{pres}({#1})}
\newcommand{\Log}[1]{\mathit{log}\;#1}
\newcommand{\EnNm}{\ensuremath{\mathit{En}}}
\newcommand{\EnName}{\EnNm\xspace} 
%
\newcommand{\InNm}{\ensuremath{\mathit{In}}}
\newcommand{\InName}{\InNm\xspace} 
%
\newcommand{\OutNm}{\ensuremath{\mathit{Out}}}
\newcommand{\OutName}{\OutNm\xspace}
%
\newcommand{\StateSpace}{\ensuremath{\mathcal{S}}}
\newcommand{\phiStates}{\ensuremath{\INV\text{-states}}\xspace}
\newcommand{\phiState}{\ensuremath{\INV\text{-state}}\xspace}
\newcommand{\AlgName}{\textsc{Minimal}}
\newcommand{\Alg}[2]{\ensuremath{\AlgName(#1,#2)}}

%

\newcommand{\LangInf}{\Lang_\text{inf}} %
\newcommand{\ArrowType}{\SelectTips{cm}{}} %



 \newcommand{\SetCategory}{\mathcal{S}\textit{et}}


\newcommand{\RLTL}{RLTL\xspace}
\newcommand{\LTL}{LTL\xspace}
\newcommand{\MuCalculus}{\ensuremath{\mu\text{-calculus}}}
%
\newcommand{\nuTL}{\ensuremath{\nu\text{TL}}}

\newcommand{\semInf}[1]{\Lang_\omega(#1)}
\renewcommand{\sem}[1]{\Lang(#1)}
\newcommand{\Aut}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\AutA}{\Aut{A}}

\newcommand{\Prop}{\textit{Prop}}


\newcommand{\PreL} [1]{\ensuremath{\!\!\phantom{.}^{-}#1}}
\newcommand{\PostL}[1]{\ensuremath{#1^{-}}}
\newcommand{\PreR} [1]{\ensuremath{\phantom{.}^{+}#1}}
\newcommand{\PostR}[1]{\ensuremath{#1^{+}}}
\newcommand{\NoMove}[1]{{\ensuremath{#1^{0}}}}
\newcommand{\BasicProp}{\Bool(\Prop)}
\newcommand{\BminusProp}{\PostL{\Bool}(\Prop)}
\newcommand{\Segment}[3]{(#1,#2,#3)}
\newcommand{\Inv}[1]{\ensuremath{#1^{-1}}}
%\newcommand{\Segment}[3]{#1[#2,#3]}
\newcommand{\Pointed}[2]{(#1,#2)}
%\newcommand{\Pointed}[2]{#1^{#2}}
\newcommand{\NotFirst}{\ensuremath{\mathit{notfirst}}}
\newcommand{\First}{\ensuremath{\mathit{first}}}

\newcommand{\modelsLTL}{\models_{\textsc{LTL}}}



==> figs/ipe/latex/figures/figures.tex <==
%\UseComputerModernTips

\newcommand{\ST}[1]{**[F-]{\texttt{#1}}}
\newcommand{\PROC}[1]{**[F-:<40pt>]{\textit{#1}}}
\newcommand{\EmbeddedAppsST}{
  \ST{\begin{tabular}{c}Embedded\\Application\\(C sources)\end{tabular}}}
\newcommand{\DirectST}{
  \PROC{\begin{tabular}{c}\phantom{A}\\\Direct\\\phantom{a} \end{tabular}}}
\newcommand{\InstrumentedSourcesST}{
  \ST{\begin{tabular}{c}Instrumented\\Annotated\\C sources\end{tabular}}}
\newcommand{\RuntimeManagerST}{
  \PROC{\begin{tabular}{c}\Direct\\Runtime\\Manager\end{tabular}}}
\newcommand{\CompileLinkST}{
  \PROC{\begin{tabular}{c}Compile\\Link\end{tabular}}}
\newcommand{\EmbeddedAppExecST}{
  \ST{\begin{tabular}{c}Embedded\\Application\\(executable)\end{tabular}}}




\newcommand{\FlowFig}{
  {\scriptsize
   \xymatrix@W=4.5em @H=4em @R=0em @C=3em {
     & & \RuntimeManagerST \ar[dr] & & \\
     \EmbeddedAppsST\ar[r] & \DirectST\ar[ur]\ar[dr] & & 
     \CompileLinkST \ar[r] & \EmbeddedAppExecST\\
     & & \InstrumentedSourcesST \ar[ur] & & \\
   }}
}
  
\newcommand{\Queue}[1]{**[F-]{\textrm{#1}}}
\newcommand{\Proc}[1]{**[F-:<50pt>]{\textit{#1}}}
%\newcommand{\Proc}[1]{*++[o][F-]{\textit{#1}}}

\newcommand{\AdhocFig}{
  {\scriptsize
   \xymatrix@W=4em @H=1.5em @R=1.3em @C=5em {
                              & \Proc{user}\ar[dl] & \Queue{user}\ar[l] &  \\
     \Queue{input}\ar[r] & \Proc{router}\ar[ur]\ar[r]\ar[dr] & \Queue{broadcast}\ar[dr] & \\
     \Proc{generator}\ar[u] & \Proc{sender}\ar[ur] & \Queue{output}\ar[l] & \Proc{delay}\ar[l]
  }
}}

==> figs/ipe/latex/macros.tex <==
\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother

% \newcommand{\mymid}{\mathbin{\mid}}
% \newcommand{\Power}[3]{{#2}\!\mymid\!{#1}\rangle\!\rangle{#3}}
% \newcommand{\WeakPower}[3]{{#2}\mymid\!{#1}\rangle{#3}} %warning: not dual power!!
% \newcommand{\PowerSub}[3]{{#2}\mymid{#1}\rangle\!\rangle{#3}}
% \newcommand{\WeakPowerSub}[3]{{#2}\mymid{#1}\rangle{#3}} %warning: not dual power!!

\newcommand{\Always}{\LTLsquare}
%\newcommand{\Always}{\mathbf{G}}
\newcommand{\Event}{\LTLdiamond}
\newcommand{\Eventually}{\Event}
\newcommand{\Next}{\LTLcircle}
\newcommand{\Prev}{\LTLcircleminus}
\newcommand{\Previously}{\Prev}
\newcommand{\PrevNoFirst}{\LTLcircletilde}
\newcommand{\Before}{\PrevNoFirst}
\newcommand{\HasAlwaysBeen}{\LTLsquareminus}
\newcommand{\SoFar}{\HasAlwaysBeen}
\newcommand{\Once}{\LTLdiamondminus}
\newcommand{\Since}{\mathbin{\mathcal{S}}}
\newcommand{\BackTo}{\mathbin{\mathcal{B}}}
\newcommand{\WeakPrev}{\LTLcircletilde}
\renewcommand{\Until}{\mathbin{\mathcal{U}}}
\newcommand{\WaitFor}{\mathbin{\mathcal{W}}}


%\newenvironment{proposition}{\theoremlike{Proposition}}{\par\medskip}

\newcommand{\val}[1]{\ensuremath{[\![ #1 ]\!]}}

\newcommand{\der}[1]{\ensuremath{\;\;{\mathop{{ %
            \longrightarrow}}\limits^{{#1}}}\!}\;\;} %

\newcommand{\Der}[1]{\ensuremath{\rightarrow_{#1}}} %
\newcommand{\notDer}[1]{\ensuremath{\not\rightarrow_{#1}}} %
%\newcommand{\notDer}[1]{\ensuremath{\;\;\not\rightarrow_{#1}\;\;}} %


\newcommand \tpl[1]{\langle #1 \rangle}


\newcommand{\LTL}{\textsf{LTL}\xspace}
\newcommand{\ForSpec}{\textsf{ForSpec}\xspace}

\newcommand{\SVA}{\textsf{SVA}\xspace}
\newcommand{\VLTL}{\textsf{VLTL}\xspace}
\newcommand{\RLTL}{\textsf{RLTL}\xspace}
%\newcommand{\RE}{\textsf{RE}\xspace}
\newcommand{\NVPA}{\textsf{NVPA}\xspace}
\newcommand{\VPA}{\textsf{VPA}\xspace}
\newcommand{\NFA}{\textsf{NFA}\xspace}
\newcommand{\VPL}{\textsf{VPL}\xspace}
\newcommand{\CARET}{\textsf{CaRet}\xspace}
\newcommand{\VPLs}{\textsf{VPL}s\xspace}
\newcommand{\VRL}{\textsf{VRL}\xspace}
\newcommand{\VRE}{\textsf{VRE}\xspace}
\newcommand{\EMSO}{\textsf{MSO$_{\mu}$}\xspace}
\newcommand{\MSO}{\textsf{MSO}\xspace}
\newcommand{\FO}{\textsf{FO}\xspace}
\newcommand{\EFO}{\textsf{FO}$_{\mu}$\xspace}
\newcommand{\XML}{\textsf{XML}\xspace}
%\newcommand{\ETL}{\textsf{ETL}\xspace}
\newcommand{\PDL}{\textsf{PDL}\xspace}
\newcommand{\AJA}{\textsf{AJA}\xspace}
\newcommand{\AJT}{\textsf{AJT}\xspace}
\newcommand{\SAJA}{\textsf{SAJA}\xspace}
\newcommand{\MAJA}{\textsf{MAJA}\xspace}
\newcommand{\AFA}{\textsf{AFA}\xspace}
\newcommand{\AVPA}{\textsf{AVPA}\xspace}
\newcommand{\PSL}{\textsf{PSL}\xspace}

\newcommand{\NWTL}{\textsf{NWTL}\xspace}
\newcommand{\NWTLPLUS}{\textsf{NWTL}$^{+}$\xspace}


\newcommand{\TWOEXPTIME}{\textsf{2-EXPTIME}\xspace}
\newcommand{\EXPTIME}{\textsf{EXPTIME}\xspace}
\newcommand{\PTIME}{\textsf{PTIME}\xspace}

\newcommand{\WM}{\ensuremath{\mathit{WM}}}
\newcommand{\MR}{\ensuremath{\mathit{MR}}}
\newcommand{\MC}{\ensuremath{\mathit{MC}}\xspace}
\newcommand{\SWM}{\ensuremath{\mathit{MWM}}\xspace}
\newcommand{\Pu}{\ensuremath{\mathcal{P}}}
\newcommand{\Lang}{\ensuremath{\mathcal{L}}}
\newcommand{\Au}{\ensuremath{\mathcal{A}}}
\newcommand{\Gam}{\ensuremath{\mathcal{G}}}
\newcommand{\Tu}{\ensuremath{\mathcal{T}}}
\newcommand{\Stratum}{\ensuremath{\mathcal{S}}}
\newcommand{\RejMain}{\ensuremath{\bot_\MainStates}}
\newcommand{\RejSec}{\ensuremath{\bot_\SecStates}}

%%%%
%%%% The following three macros are confusing with MainStates and SecStates
%%%%
\newcommand{\Msubst}{$M$-substitution\xspace} % M-substitution CHANGE FONT
\newcommand{\Mclosure}{$M$-closure\xspace}    %
\newcommand{\Sclosure}{$S$-closure\xspace}    %

\newcommand{\Region}{\ensuremath{\mathcal{R}}}

%\newcommand{\MainStates}{\ensuremath{\textit{M}}}
%\newcommand{\MainStates}{\ensuremath{M}}
\newcommand{\MainStates}{\ensuremath{\mathsf{M}}}
%\newcommand{\SecStates}{\ensuremath{\textit{S}}}
%\newcommand{\SecStates}{\ensuremath{S}}
\newcommand{\SecStates}{\ensuremath{\mathsf{S}}}
%\newcommand{\FamStratum}{\ensuremath{\mathfrak{F}}}
\newcommand{\FamStratum}{\ensuremath{\mathsf{F}}}
\newcommand{\Acc}{\ensuremath{\textit{Acc}}}
\newcommand{\Inf}{\ensuremath{\textit{Inf}}}
\newcommand{\SF}{\ensuremath{\textit{SF}}}
\newcommand{\Model}{\ensuremath{\textit{X}}}



\newcommand{\Stilde}{\widetilde{\Sigma}\xspace}
\newcommand{\Scall}{\Sigma_{\mathit{call}}}
\newcommand{\call}{{\mathit{call}}}
\newcommand{\ret}{{\mathit{ret}}}
\newcommand{\intA}{{\mathit{int}}}
\newcommand{\Sret}{\Sigma_{\mathit{ret}}}
\newcommand{\Sint}{\Sigma_{\mathit{int}}}

\newcommand{\Nat}{\mathbb{N}}



\newcommand{\SubstOp}[1]{\mathrel{\curvearrowleft_{#1}}}
\newcommand{\SubstBox}{\SubstOp{\Box}}
\newcommand{\MClos}[2]{#1^{\SubstOp{#2}}}
\newcommand{\LangClos}{\MClos{\Lang}{\Box}}
\newcommand{\SClos}[2]{{#1}^{\circlearrowleft_{#2}}}
\newcommand{\SClosure}[1]{\SClos{#1}{\Box}}
\newcommand{\LangSClos}{\SClos{\Lang}{\Box}}

\newcommand{\caller}{\mathsf{c}}
\newcommand{\down}{\mathsf{+}}
\newcommand{\abs}{\mathsf{a}}
\newcommand{\absExt}{\mathsf{ea}}
\newcommand{\PosBool}{\ensuremath{\mathcal{B}^{+}}}

%\newcommand{\dirUp}{\ensuremath{\uparrow}}
\newcommand{\dirUp}{\ensuremath{\leftarrow}}
%\newcommand{\dirDown}{\ensuremath{\downarrow}}
\newcommand{\dirDown}{\ensuremath{\rightarrow}}
%\newcommand{\dirUpAbs}{\ensuremath{\uparrow^{\abs}}}
\newcommand{\dirUpAbs}{\ensuremath{\curvearrowleft}}
%\newcommand{\dirDownAbs}{\ensuremath{\downarrow_{\abs}}}
\newcommand{\dirDownAbs}{\ensuremath{\curvearrowright}}
%\newcommand{\dirDownAbsExt}{\ensuremath{\downarrow_{\absExt}}}
%\newcommand{\dirDownAbsExt}{\ensuremath{\curvearrowright_{\mkern-15.2mu\raisebox{.30em}{$\phantom{.}_{\bullet}$}}}}
\newcommand{\dirDownAbsExt}{\ensuremath{\curvearrowright_{\mkern-8.5mu{\bullet}}}}
%\newcommand{\dirUpAbsExt}{\ensuremath{\uparrow^{\absExt}}}
%\newcommand{\dirUpAbsExt}{\ensuremath{\curvearrowleft_{\mkern-30.2mu\raisebox{.30em}{$\phantom{.}_{\bullet}$}}}}
\newcommand{\dirUpAbsExt}{\ensuremath{\phantom{.}_\bullet{\mkern-8.2mu\curvearrowleft}}}

\newcommand{\DIR}{\textit{DIR}}
\newcommand{\Trans}{\texttt{t}}
\newcommand{\Moves}{\textit{Moves}}
%\newcommand{\dir}{\textit{dir}}
\newcommand{\SUCC}{\mathsf{succ}}
\newcommand{\NULL}{\mathsf{\bot}}
\newcommand{\acc}{\textit{acc}}
\newcommand{\rej}{\textit{rej}}
\newcommand{\rank}{\textit{rank}}
\newcommand{\widt}{\textit{width}}

\newcommand{\DefinedAs}{\,\stackrel{\text{def}}{=}\,}

%\newcommand{\DefOR}{\ensuremath{\;\;\;\big|\;\;\;}}
\newcommand{\DefORmini}{\ensuremath{\;\big|\;}}

\newcommand{\details}[1]{}

%%%%%% Temporal Modalities %%%%%%%%%%%%%%

\newcommand{\true}{\ensuremath{\textup{\texttt{true}}}}
\newcommand{\false}{\ensuremath{\textup{\texttt{false}}}}
\newcommand{\Power}[3]{\mathrel{{#1}|{#2}\rrangle{#3}}}
\newcommand{\Norm}[1]{\ensuremath{\|{#1}\|}}
\newcommand{\WeakPower}[3]{\mathrel{{#1}|{#2}\rangle{#3}}}
\newcommand{\PastPower}[3]{\mathrel{{#1}\llangle{#2}|{#3}}}
\newcommand{\PastWeakPower}[3]{\mathrel{{#1}\langle{#2}|{#3}}}
%\newcommand{\Next}{\ensuremath{\bigcirc}}
\newcommand{\Seq}{\ensuremath{;}}
%\newcommand{\Previous}{\ensuremath{{\mathrlap{\bigcirc}\,\minus\,}}}
\newcommand{\Previous}{\Prev}
%\newcommand{\until}{{\sf U}}
\newcommand{\until}{\Until}
%\newcommand{\since}{{\sf S}}
\newcommand{\since}{\Since}
%\newcommand{\sometimes}{\lozenge}
%\newcommand{\always}{\square}
\newcommand{\always}{\Always}

\newcommand{\comp}[1]{\ensuremath{\overline{#1}}} % complement automaton
\newcommand{\dual}[1]{\ensuremath{\widetilde{#1}}} % dualization

\newcommand{\Outcm}{c\,b\,r}
\newcommand{\UOutcm}{\underline{\Outcm}}

\newenvironment{changemargin}[2]{%
  \begin{list}{}{%
    \setlength{\topsep}{0pt}%
    \setlength{\leftmargin}{#1}%
    %\setlength{\footnotewidth}{#1}%
    \setlength{\rightmargin}{#2}%
    \setlength{\textheight}{21cm}%
   \setlength{\topmargin}{0cm}
   \setlength{\listparindent}{\parindent}%
    \setlength{\itemindent}{\parindent}%
    \setlength{\parsep}{\parskip}%
  }
  \item[]}{\end{list}}


\newcommand{\push}{\textit{push}}
\newcommand{\Regions}{\ensuremath{\textit{REG}}}
\newcommand{\pop}{\textit{pop}}
%\newcommand{\pending}{\ensuremath{\texttt{pending}}}

\newcommand{\Bu}{\ensuremath{\textsf{B}}}
\newcommand{\Co}{\ensuremath{\textsf{C}}}

\newcommand{\alphaANY}{\ensuremath{\alpha_{\mathit{ONE}}}}

%%%% ATTENTION HERE: DON'T USE OLD DEFINITION IN FSTTCS CLASS iS treated as a section %%%%
\newcommand{\myparagraph}[1]{\paragraph{\textup{\textbf{#1}}}}
%\newcommand{\myparagraph}[1]{\noindent\textbf{#1}}

\newcommand{\myparagraphApp}[1]{\vspace{0.5em}\noindent\textup{\textbf{#1}}}

\newcommand{\qin}{\ensuremath{q_{\textit{in}}}}

==> figs/ipe/latex/macros/altba.tex <==
\newcommand{\var}{{\mathcal{X}}}
\newcommand{\posform}[1]{\mathcal{B}^+(#1)}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> figs/ipe/latex/macros/automata.tex <==
%\newcommand{\AutNode}[1]{*+[F-:<3pt>]{#1}}
\newcommand{\AutNode}[1]{*+[o][F-]{#1}}
\newcommand{\AutFinalNode}[1]{*+[o][F=]{#1}}

==> figs/ipe/latex/macros/colors.tex <==
\newcommand{\VLC}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\VRC}[1]{\textcolor{darkred}{#1}}
\newcommand{\emphC}[1]{\textcolor{red}{#1}}
\newcommand{\GR}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\RD}[1]{\textcolor{darkred}{#1}}
\newcommand{\BL}[1]{\textcolor{darkblue}{#1}}
\newcommand{\ORN}[1]{\textcolor{darkorange}{#1}}
\newcommand{\ColRE}[1]{\ORN{#1}}
\newcommand{\ColTL}[1]{\RD{#1}}
\newcommand{\ColAUT}[1]{\BL{#1}}
\newcommand{\ColL}[1]{\GR{#1}}

\newcommand{\Cr}{\ColRE{r}}
\newcommand{\Cs}{\ColRE{s}}
\newcommand{\Cx}{\ColTL{x}}
\newcommand{\Cy}{\ColTL{y}}
\newcommand{\Cz}{\ColTL{z}}
\newcommand{\spc}{\hspace{2em}}
\newcommand{\one}{\ColRE{\textit{one}}}
\newcommand{\mwm}{\ColRE{\textit{mwm}}}
\newcommand{\wm}{\ColRE{\textit{wm}}}
\newcommand{\mr}{\ColRE{\textit{mr}}}
\newcommand{\ttrue}{\ColTL{\texttt{true}}}
\newcommand{\Henceforth}{\ColTL{\textbf{G}}}
\newcommand{\ABS}{\ColRE{\textit{abs}}}
\newcommand{\CALLER}{\ColRE{\textit{caller}}}
\newcommand{\sumOne}{\ColRE{\textit{sum1}}}
\newcommand{\sumTwo}{\ColRE{\textit{sum2}}}
\newcommand{\Aut}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\AutA}{\Aut{A}}


==> figs/ipe/latex/macros/direct.tex <==
\newcommand{\Direct}{\textsc{Direct}\xspace}
\newcommand{\into}{\rightarrow}

%%%% FIGURE WITH 2 PROGRAMS
\begin{SaveVerbatim}[fontfamily=courier]{Thread-1}
1  void infa(void)  {
2    while (1) {
3      if (exp) {
4        mutex_lock(b);
5        mutex_lock(a);
6        // critical sect
7        mutex_unlock(a);
8        mutex_unlock(b);
9     } else {
10       mutex_lock(c);
11       mutex_lock(a);
12       // critical sect
13       mutex_unlock(a);
14       mutex_unlock(c);
15     }
16   }
17 }
\end{SaveVerbatim}

\begin{SaveVerbatim}[fontfamily=courier]{Thread-2}
21 void infb(void) {
22   while (1) {
23     mutex_lock(a);
24     mutex_lock(b);
25     // critical sect
26     mutex_unlock(b);
27     mutex_unlock(a);
28   }
29 }
\end{SaveVerbatim}

%%%%% TRACE OF DINING PHILOSPHERS
\newcommand{\DiningTrace}{
\begin{tabular}{|l||l|l|l|l|l|l|l|l|l|}
        \hline
$\textit{State}$ & $\textit{Thrd}$ & 
\multicolumn{5}{|c|}{\textit{Philosopher threads}} & \textit{Res} & \textit{Res} & $\textit{(c)alls/}$ \\
$\textit{no.}$ & $\textit{id}$ & $T_0$ & $T_1$ & $T_2$ & $T_3$ & $T_4$ & $\textit{values}$ & $\textit{held}$ & $\textit{(r)ets}$ \\
        \hline \hline
$1$  & $3$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 1)$ &  $(0, 0)$ & $(0,0,0,1,1)$ & $()$ & $c$ \\
\rowcolor[rgb]{0.90,0.99,0.90}$2$  & $3$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 1)$ &  $(0, 0)$ & $(0,0,0,0,1)$ & $(3)$ & $r$ \\
$3$  & $3$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 0)$ & $(0,0,0,0,1)$ & $(3)$ & $c$ \\
$4$  & $4$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 0)$ & $(0,0,0,0,1)$ & $()$ & $r$ \\
\rowcolor[rgb]{0.99,0.90,0.90}$5$  & $4$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 1)$ & $(0,0,0,0,1)$ & $()$ & $c$ \\
\rowcolor[rgb]{0.99,0.80,0.80}$6$  & $4$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 2)$ &  $(0, 1)$ & $(0,0,0,0,0)$ & $(4)$ & $r$ \\
$\ldots$  & $\ldots$ &  &  &  &  &  & & & \\
$16$ & $4$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 2)$ & $(0,0,0,0,0)$ & $(4)$ & $r$ \\
\rowcolor[rgb]{0.90,0.70,0.70}$17$ & $4$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ &  $(0, 3)$ & $(0,0,0,0,0)$ & $(4)$ & $c$ \\
        \hline
\end{tabular}
}



==> figs/ipe/latex/macros/enriched.tex <==
%%%%% %%%%% 1. for the enriched paper %%%%%
%\newcommand{\F}{\mathsf{F}} %\newcommand{\T}{\mathsf{T}}
%\newcommand{\F}{\mathbf{false}}
%\newcommand{\T}{\mathbf{true}}
%\newcommand{\true}{\T}
%\providecommand*{\Always}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Always}{\LTLsquare}
%\providecommand*{\Event}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Event}{\LTLdiamond}
%\providecommand*{\Next}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Next}{\LTLcircle}
%\newcommand{\Prev}{\LTLcircleminus}
%\newcommand{\PrevNoFirst}{\LTLcircletilde}
%\newcommand{\HasAlwaysBeen}{\LTLsquareminus}
%\providecommand*{\Once}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Once}{\LTLdiamondminus}
%\providecommand*{\Since}{} %Ale: to compile with cesar-llncs
%\renewcommand{\Since}{\mathbin{\mathcal{S}}}
%\providecommand*{\BackTo}{} %Ale: to compile with cesar-llncs
%\renewcommand{\BackTo}{\mathbin{\mathcal{B}}}
%\newcommand{\WeakPrev}{\LTLcircletilde}


\newcommand{\ORsym}{{\scriptstyle{\pmb{+}}}}
\newcommand{\SEQsym}{{\scriptstyle{\cdot}}}
\newcommand{\ANDsym}{{\scriptstyle{\pmb{|}}}}
\newcommand{\STARsym}{*}
\newcommand{\EXPsym}{\widehat{\;\phantom{\cdot}\;}}
\newcommand{\POWsym}{\EXPsym}
\newcommand{\DPOWsym}{\_}
\newcommand{\NEGsym}{\overline{\;\phantom{\cdot}\;}}
%\newcommand{\INF}[1]{\overset{\infty}{#1}}
\newcommand{\INF}[1]{\widehat{#1}}
%\newcommand{\ORsymInf}{\INF{\ORsym}}
\newcommand{\ORsymInf}{\oplus}
%\newcommand{\ANDsymInf}{\INF{\ANDsym}}
\newcommand{\ANDsymInf}{\oslash}
%\newcommand{\SEQsymInf}{\INF{\SEQsym}} 
\newcommand{\SEQsymInf}{\odot} 
\newcommand{\OR}{\mathrel{+}}
\newcommand{\AND}{\mathrel{|}} 
\newcommand{\SEQ}{\mathrel{\cdot}}
%\newcommand{\ORInf}{\mathrel{\INF{\scriptstyle{+}}}}
\newcommand{\ORInf}{\mathrel{\oplus}}
%\newcommand{\ANDInf}{\mathrel{\INF{\scriptstyle{|}}}}
\newcommand{\ANDInf}{\mathrel{\oslash}}
%\newcommand{\SEQInf}{\mathrel{\INF{\scriptstyle{\cdot}}}}
\newcommand{\SEQInf}{\mathrel{\odot}}

\newcommand{\uSTAR}{^\STARsym} %unary star
\newcommand{\bSTAR}{\mathrel{\STARsym}} %unary star
\newcommand{\STAR}{\uSTAR} \newcommand{\CIRC}{\mathrel{\circ}}
%\newcommand{\EnrichedRE}{E$\omega${}RE\xspace}
\newcommand{\EnrichedRE}{\ensuremath{\textup{EnRE}}\xspace}
\newcommand{\EnRE}{\EnrichedRE}
\newcommand{\VeryEnrichedRE}{kE$\omega${}RE\xspace}
%\newcommand{\Vars}{\mathcal{V}}
\newcommand{\ElemRE}{\ensuremath{\textup{ElemRE}}\xspace}
%\newcommand{\Bool}{\mathcal{B}}
\newcommand{\wRE}[1]{\ensuremath{\omega\text{RE}(#1)}}
\newcommand{\finRE}[1]{\ensuremath{\text{RE}(#1)}}
\newcommand{\RE}{\textup{RE}\xspace} % regular expressions
\newcommand{\ERE}{\textup{ERE}\xspace} % Extended Regular Expressions RE(+,*,;,|,~,[w]) 
\newcommand{\SERE}{\textup{SERE}\xspace} %Semi-Extended Regular Expressions RE(+,*,;,|, ,[w])

\newcommand{\SigmaElem}{\Sigma_\text{elem}}
\newcommand{\SigmaEnriched}{\Sigma_\text{rich}}
\newcommand{\SigmaEnrichedInf}{\Sigma^{\omega}_\text{rich}}
\newcommand{\SigmaRegexp}{\Sigma_\text{regexp}}

\newcommand{\NBW}{NBW\xspace} % non-deterministic B\"uchi automata on words 
\newcommand{\DBW}{DBW\xspace} % deterministic B\"uchi automata on words 
\newcommand{\ABW}{ABW\xspace} % alternating B\"uchi automata on words 
\newcommand{\BABW}{BABW\xspace} %
\newcommand{\ETL}{\text{ETL}\xspace} % Extended Temporal Logic ETL
\newcommand{\ETLr}{\ensuremath{\text{ETL}_r}\xspace} % ETL (regular condition) 
\newcommand{\ETLl}{\ensuremath{\text{ETL}_l\xspace}} % ETL (loop condition) 
\newcommand{\ETLf}{\ensuremath{\text{ETL}_f\xspace}}
% ETL (finite condition)
\newcommand{\ETLa}{\ensuremath{\text{ETL}_a\xspace}} % ETL(alternating condition)
\newcommand{\ETLta}{\ensuremath{\text{ETL}_2a}\xspace} % ETL (two way alternating condition) 
\newcommand{\Release}{\mathbin{\mathcal{R}}}

\newcommand{\ALL}{\ensuremath{\mathbf{all}}\xspace}

%\newcommand{\Alphabet}{\Gamma}
\newcommand{\Alphabet}{\Sigma}

\newcommand{\Eqs}{\mathcal{E}}


\newcommand{\DefOR}{\ensuremath{\;\;\;\big|\;\;\;}}
\renewcommand{\SEQsym}{\ensuremath{;}}
\renewcommand{\SEQ}{\mathrel{\SEQsym}}

\newcommand{\REOR}{+}
\newcommand{\RESEQsym}{\ensuremath{;}}
\newcommand{\RESeq}{\mathrel{\RESEQsym}}
\newcommand{\REStar}{*}


==> figs/ipe/latex/macros/general.tex <==
\newcommand\Def[2][]{%                        % F"ur Definitionen 
  \def\temp{#1}%                              % die in den Index sollen
  \ifx\temp\empty%
    \def\temp{#2}%
  \fi%
%{\em\boldmath#2\unboldmath\index{\temp}}}
{\em#2\index{\temp}}}

\newcommand{\N}{\mathbb{N}}

\newcommand{\onlyWithComplement}[1]{}

%\newcommand{\pos}{\textit{pos}}
%\newcommand{\Pos}{\textit{Pos}}
\newcommand{\pos}{\omega}
\newcommand{\Pos}{\omega}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> figs/ipe/latex/macros/macros.tex <==
\input{macros/general}
\input{macros/enriched}
\input{macros/rules}
\input{macros/altba}
\input{macros/automata}
\input{macros/direct}
\input{macros/colors}

==> figs/ipe/latex/macros/rules.tex <==

%\newcommand{\AccSym}{\uparrow}
% \newcommand{\AccSym}{\tick}
%%\RequirePackage{pifont}
%% \newcommand{\tick}{\ding{51}}
%% \newcommand{\AccSym}{\tick}

\RequirePackage{amssymb}
\newcommand{\AccSym}{\surd}


%\newcommand{\RejSym}{\downarrow}
\RequirePackage{pifont}
%\newcommand{\RejSym}{\text{\ding{53}}}
\newcommand{\RejSym}{\,\mathsf{x}\,}

% \newcommand{\ACC}[1]{\ensuremath{\overset{#1}{\AccSym}}}
 \newcommand{\ACC}[1]{\ensuremath{{\AccSym}\hspace{-0.7em}{\overset{#1}{\text{\phantom{x}}}}}}
 \newcommand{\ACCa}{\ACC{s}}
 \newcommand{\REJ}[1]{\ensuremath{\overset{#1}{\RejSym}}}
 \newcommand{\REJa}{\REJ{s}}
 \newcommand{\DER}[1]{\ensuremath{\overset{#1}{\Into}}}
 \newcommand{\DERa}{\DER{s}}

 \newcommand{\BasicAcceptRuleA}{\ell \ACCa\;\;\text{(if $s\models \ell$)}}
 \newcommand{\BasicAcceptRuleB}{\ell \REJa\;\;\text{(if $s\nmodels \ell$)}}
 \newcommand{\BasicNextRule}{\ell \DERa \F}


 \newcommand{\ORAcceptRuleA}{
   \AxiomC{$x\ACCa$}
   %\LeftLabel{\ORAcceptRuleALabel}
   \UnaryInfC{$x \OR y \ACCa$}
   \DisplayProof
 }
 \newcommand{\ORAcceptRuleB}{
   \AxiomC{$y\ACCa$}
   %\LeftLabel{\ORAcceptRuleALabel}
   \UnaryInfC{$x \OR y \ACCa$}
   \DisplayProof
 }
 \newcommand{\ORAcceptRuleC}{
      \AxiomC{$x\REJa$}
      \AxiomC{$y\REJa$}
      %\LeftLabel{\ORAcceptRuleALabel}
      \BinaryInfC{$x \OR y \REJa$}
      \DisplayProof
 }
 \newcommand{\OrNextRule}{
      \AxiomC{$x\DERa x'$}
      \AxiomC{$y\DERa y'$}
      %\LeftLabel{\ORAcceptRuleALabel}
      \BinaryInfC{$x \OR y \DERa x' \OR y'$}
      \DisplayProof
 }

 \newcommand{\AndAcceptRuleA}{
   \AxiomC{$x\REJa$}
   %\LeftLabel{\ORAcceptRuleALabel}
   \UnaryInfC{$x \AND y \REJa$}
   \DisplayProof
   
 }
 \newcommand{\AndAcceptRuleB}{
   \AxiomC{$y\REJa$}
   %\LeftLabel{\ORAcceptRuleALabel}
   \UnaryInfC{$x \AND y \REJa$}
   \DisplayProof
}
\newcommand{\AndAcceptRuleC}{
  \AxiomC{$x\ACCa$}
  \AxiomC{$y\ACCa$}
  %\LeftLabel{\ORAcceptRuleALabel}
  \BinaryInfC{$x \AND y \ACCa$}
  \DisplayProof
}
\newcommand{\AndNextRule}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  %\LeftLabel{\ORAcceptRuleALabel}
  \BinaryInfC{$x \AND y \DERa x' \AND y'$}
  \DisplayProof
}

\newcommand{\SeqAcceptRule}{
  x \SEQ y \REJa
}

\newcommand{\SeqNextRuleA}{
  \AxiomC{$x\ACCa$}
  \AxiomC{$x\DERa x'$}
  %\LeftLabel{\ORAcceptRuleALabel}
  \BinaryInfC{$x \SEQ y \DERa x'\SEQ y \OR y$}
  \DisplayProof
}
\newcommand{\SeqNextRuleB}{
  \AxiomC{$x\REJa$}
  \AxiomC{$x\DERa x'$}
  %\LeftLabel{\ORAcceptRuleALabel}
  \BinaryInfC{$x \SEQ y \DERa x'\SEQ y$}
  \DisplayProof
}

\newcommand{\PowAcceptRuleA}{
  \AxiomC{$y\ACCa$}
  \UnaryInfC{$x^z y \ACCa$}
  \DisplayProof
}
\newcommand{\PowAcceptRuleB}{
  \AxiomC{$y\REJa$}
  \UnaryInfC{$x^z y \REJa$}
  \DisplayProof
}
\newcommand{\PowNextRuleA}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  \AxiomC{$z\DERa z'\;\;\;\;z\REJa$}
  \TrinaryInfC{$x^z y \DERa y' \OR (x' \AND (z' \SEQ x^z y))\text{\phantom{$\OR x^z y$}}$}
  \DisplayProof
}
\newcommand{\PowNextRuleB}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  \AxiomC{$z\DERa z'\;\;\;\;z\ACCa$}
  \TrinaryInfC{$x^z y \DERa y' \OR (x' \AND (z' \SEQ x^z y \OR x^z y))$}
  \DisplayProof
}

\newcommand{\DualPowAcceptRuleA}{
  \AxiomC{$y\REJa$}
  \UnaryInfC{$x_z y \REJa$}
  \DisplayProof
}
\newcommand{\DualPowAcceptRuleB}{
  \AxiomC{$y\ACCa$}
  \AxiomC{$x\ACCa$}
  \BinaryInfC{$x_z y \ACCa$}
  \DisplayProof
}
\newcommand{\DualPowAcceptRuleC}{
  \AxiomC{$y\ACCa$}
  \AxiomC{$x\REJa$}
  \BinaryInfC{$x_z y \REJa$}
  \DisplayProof
}



\newcommand{\DualPowNextRuleA}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  \AxiomC{$z\DERa z'\;\;\;\;z\REJa$}
  \TrinaryInfC{$x_z y \DERa y' \AND (x' \OR (z' \SEQ x_z y))\text{\phantom{$\OR x^z y$}}$}
  \DisplayProof
}
\newcommand{\DualPowNextRuleB}{
  \AxiomC{$x\DERa x'$}
  \AxiomC{$y\DERa y'$}
  \AxiomC{$z\DERa z'\;\;\;\;z\ACCa$}
  \TrinaryInfC{$x_z y \DERa y' \AND (x' \OR (z' \SEQ x_z y \OR x_z y))$}
  \DisplayProof
}

\newcommand{\EquationAcceptRuleA}{
  \AxiomC{$\phi(x_1,\ldots) \ACCa$}
  \UnaryInfC{$\phi(x_1,\ldots) \ACCa_\Eqs$}
  \DisplayProof 
}

\newcommand{\EquationAcceptRuleB}{
  \AxiomC{$\phi(x_1,\ldots) \REJa$}
  \UnaryInfC{$\phi(x_1,\ldots) \REJa_\Eqs$}
  \DisplayProof 
}

\newcommand{\EquationNextRule}{ 
  \AxiomC{$\phi(x_1,\ldots,x_n) \DERa \phi'(x_1,\ldots,x_n)$} 
  \UnaryInfC{$\phi \DERa_\Eqs
    \phi'(\phi_{x_1},\ldots,\phi_{x_n})$} 
  \DisplayProof 
}


==> figs/ipe/latex/programs.tex <==
\newcommand{\RefFigListClass}{\ref{fig:programs}(a)\xspace}
\newcommand{\RefFigMGC}      {\ref{fig:programs}(b)\xspace}
\newcommand{\RefFigSearch}   {\ref{fig:programs}(c)\xspace}
\newcommand{\RefFigLocate}   {\ref{fig:programs}(d)\xspace}
\newcommand{\RefFigAdd}      {\ref{fig:programs}(e)\xspace}
\newcommand{\RefFigRemove}   {\ref{fig:programs}(f)\xspace}

\newcommand{\RefFigListClassGhost}{\ref{fig:programs:ghost}(a)\xspace}
\newcommand{\RefFigLocateGhost}		{\ref{fig:programs:ghost}(b)\xspace}
\newcommand{\RefFigAddGhost}			{\ref{fig:programs:ghost}(c)\xspace}
\newcommand{\RefFigRemoveGhost}		{\ref{fig:programs:ghost}(d)\xspace}

\newcommand{\FigLabel}[1]{\multicolumn{1}{c}{#1}}
\newcommand{\FigLabelWide}[1]{\multicolumn{3}{c}{#1}}

%
% Figures for data structure
%

\begin{SaveVerbatim}{list-data}
class List {
     Node list;
}
\end{SaveVerbatim}

\begin{SaveVerbatim}{list-data-space}
class List {
     Node list;

}
\end{SaveVerbatim}


\begin{SaveVerbatim}{node-data}
class Node {
     Value val;
     Node next;
     Lock lock;
}
\end{SaveVerbatim}

\newcommand{\DataStructuresBody}{
  \begin{tabular}{l}
    \renewcommand{\arraystretch}{0.4}
    $\begin{array}{l}
      \class \: \List \: \{ \\
      \mhs \Node \: \tList ;\\
      \}
    \end{array}$ \\ \\ \\
    \renewcommand{\arraystretch}{0.4}
    $\begin{array}{l}
      \class \: \Node \: \{ \\
      \mhs \Value \: \val ;\\
      \mhs \Node \: \tNext ;\\
      \mhs \Lock \: \lock ;\\
      \}
    \end{array}$
  \end{tabular}
}
\newcommand{\DataStructuresFig}{
\begin{minipage}[c]{3.7cm}
  \DataStructuresBody
\label{fig:listclass}
\end{minipage}
}

%
% Figures for most generate cliente "decide"
%
\newcommand{\MGCBody}{
  \begin{algorithmic}[1]
    \While {$\true$}
    \State $e := \NondetChooseElem$
    \State $\Nondet$
    \State $\left[ \begin{array}{l}
	\Call \search(e) \\
	\ProgOr \\
	\Call \add(e) \\
	\ProgOr \\
	\Call \remove(e)
      \end{array} \right]$
    \EndWhile
  \end{algorithmic}
}

\begin{SaveVerbatim}[fontfamily=courier]{mgc-prg}
0:  while true
1:     e:= NonDet();
2:     select
3:        search(e);
4:     or
5:        add(e);
6:     or
7:        remove(e);
8:  end;
\end{SaveVerbatim}

\newcommand{\MGCPrg}{
  \begin{minipage}[c]{5.0cm}
    \MGCBody
  \end{minipage}
}
\newcommand{\MGCFig}{
  \begin{minipage}[c]{4.1cm}
    \MGCBody
    \label{fig:mgc}
  \end{minipage}
}

%
% Figure for "search" 
%
\begin{SaveVerbatim}{search-prog}
20:  prev, cur := locate (e);
21:  if curr.val = e then
22:      result := true;
23:  else
24:      result := false;
25:  curr.unlock();
26:  prev.unlock();
27:  return result;
\end{SaveVerbatim}

\newcommand{\SearchBody}{
  \begin{algorithmic}[1]
    \State $\prev, \curr := \locate(e)$
    \If {$\curr.\val = e$}
    \State $\result := \true$
    \Else
    \State $\result := \false$
    \EndIf
    \State $\curr.\unlock()$
    \State $\prev.\unlock()$
    \State \tbf{return} $\result$
  \end{algorithmic}
}
\newcommand{\SearchPrg}{
  \begin{minipage}[c]{3.9cm}
    \SearchBody
  \end{minipage}
}
\newcommand{\SearchFig}{
\begin{minipage}[c]{3.9cm}
  \SearchBody
\label{fig:search}
\end{minipage}
}

%
% Figure for "locate"
%
\begin{SaveVerbatim}{locate-prog}
 9:  prev := Head;
10:  prev.lock();
11:  curr := prev.next;
12:  curr.lock();
13:  while curr.val < e do
14:      prev.unlock();
15:      prev := curr;
16:      curr := curr.next;
17:      curr.lock();
18:  end;
19:  return (prev,curr)
\end{SaveVerbatim}

\newcommand{\LocateBody}{
\begin{algorithmic}[1]
\State $\prev := \Head$
\State $\prev.\lock()$
\State $\curr := \prev.\tNext$
\State $\curr.lock()$
\While {$\curr.\val < e$}
	\State $\prev.\unlock()$
	\State $\prev := \curr$
	\State $\curr := \curr.\tNext$
	\State $\curr.\lock()$
\EndWhile
\State \tbf{return} $(\prev, \curr)$
\Statex
\end{algorithmic}
}

\newcommand{\LocatePrg}{
  \begin{minipage}[c]{3.7cm}
    \LocateBody
  \end{minipage}
}

\newcommand{\LocateFig}{
\begin{minipage}[c]{3.7cm}
  \LocateBody
\label{fig:locate}
\end{minipage}
}

%
% Figure for "add"
%
\begin{SaveVerbatim}{add-prog}
28:  prev, curr := locate(e);
29:  if curr.val != e then
30:      aux := new Node(e);
31:      aux.next := curr;
32:      prev.next := aux;
33:      result := true;
34:  else
35:      result := false;
36:  end;
37:  prev.unlock();
38:  curr.unlock();
39:  return result;
\end{SaveVerbatim}



\newcommand{\AddBody}{
\begin{algorithmic}[1]
\State $\prev, \curr := \locate(e)$
\If {$\curr.\val \neq e$}
	\State $\aux := \New \Node(e)$
	\State $\aux.\tNext := \curr$
	\State $\prev.\tNext := \aux$
	\State $\result := \true$
\Else
	\State $\result := \false$
\EndIf
\State $\prev.\unlock()$
\State $\curr.\unlock()$
\State \tbf{return} $\result$
\end{algorithmic}
}

\newcommand{\AddPrg}{
  \begin{minipage}[c]{4.1cm}
    \AddBody
  \end{minipage}
}

\newcommand{\AddFig}{
\begin{minipage}[c]{4.1cm}
  \AddBody
  \label{fig:add}
\end{minipage}
}

%
% Figure for "remove"
%
\begin{SaveVerbatim}{remove-prog}
40:  prev, curr := locate(e);
41:  if curr.val == e then
42:      aux := curr.next;
43:      prev.next := aux;
44:      result := true;
45:  else
46:      result := false;
47:  end;
48:  prev.unlock();
49:  curr.unlock();
50:  return result;
\end{SaveVerbatim}


\newcommand{\RemoveBody}{
    \begin{algorithmic}[1]
      \State $\prev, \curr := \locate(e)$
      \If {$\curr.\val = e$}
      \State $\aux := \curr.\tNext$
      \State $\prev.\tNext := \aux$
      \State $\result := \true$
      \Else
      \State $\result := \false$
      \EndIf
      \State $\prev.\unlock()$
      \State $\curr.\unlock()$
      \State \tbf{return} $\result$
      \Statex
    \end{algorithmic}
}

\newcommand{\RemovePrg}{
  \begin{minipage}[c]{3.9cm}
    \RemoveBody
  \end{minipage}
}


\newcommand{\RemoveFig}{
  \begin{minipage}[c]{3.9cm}
    \RemoveBody
    \label{fig:remove}
  \end{minipage}
}




%
% Figures for data structure
%
\newcommand{\DataStructuresGhostBody}{
	\begin{tabular}{cc}
		\renewcommand{\arraystretch}{0.4}
		$\begin{array}{l}
			\class \: \List \: \{ \\
			\mhs \Node \: \tList ;\\
			\hs{0.2} \fbox{ \begin{array}{l}
				\rgn \: r; \\
			\end{array}}\\
		\}
		\end{array}$ & \hs{2} $\begin{array}{l}
			\class \: \Node \: \{ \\
			\mhs \Value \: \val ;\\
			\mhs \Node \: \tNext ;\\
			\mhs \Lock \: \lock ;\\
		\}
	\end{array}$
	\end{tabular}
}

\newcommand{\DataStructuresGhostFig}{
\begin{minipage}[c]{6.5cm}
	\DataStructuresGhostBody
\label{fig:conclists:ghost}
\end{minipage}
}


%
% Figure for "locate" extended with ghost fields
%

\newcommand{\LocateGhostBody}{
	\begin{algorithmic}[1]
		\State $\prev := \Head$
		\State $\prev.\lock()$
		\State $\curr := \prev.\tNext$
		\State $\curr.lock()$
		\While {$\curr.\val < e$}
			\State $\prev.\unlock()$
			\State $\prev := \curr$
			\State $\curr := \curr.\tNext$
			\State $\curr.\lock()$
		\EndWhile
		\State \tbf{return} $(\prev, \curr)$
		\vspace{0.8cm}
	\end{algorithmic}
}


\newcommand{\LocateGhostFig}{
\begin{minipage}[c]{4.2cm}
	\LocateGhostBody
\label{fig:locate:ghost}
\end{minipage}
}


%
% Figure for "add" extended with ghost fields
%
\newcommand{\AddGhostBody}{
	\begin{algorithmic}[1]
		\State $\prev, \curr := \locate(e)$
		\If {$\curr.\val \neq e$}
			\State $\aux := \New \Node(e)$
			\State $\aux.\tNext := \curr$
			\State $\prev.\tNext := \aux$
			\Statex $\hs{0.7}\fbox{
				\begin{array}{l}
					l.r := l.r \cup \sreg{\aux} \\
				\end{array}}$
			\State $\result := \true$
		\Else
			\State $\result := \false$
		\EndIf
		\State $\prev.\unlock()$
		\State $\curr.\unlock()$
		\State \tbf{return} $\result$
	\end{algorithmic}
}


\newcommand{\AddGhostFig}{
\begin{minipage}[c]{4.2cm}
	\AddGhostBody
	\label{fig:add:ghost}
\end{minipage}
}


%
% Figure for "remove" extended with ghost fields
%
\newcommand{\RemoveGhostBody}{
		\begin{algorithmic}[1]
			\State $\prev, \curr := \locate(e)$
			\If {$\curr.\val = e$}
				\State $\aux := \curr.\tNext$
				\State $\prev.\tNext := \aux$
				\Statex $\hs{0.7}\fbox{
					\begin{array}{l}
						l.r := l.r - \sreg{\curr} \\
					\end{array}}$
				\State $\result := \true$
			\Else
				\State $\result := \false$
			\EndIf
			\State $\prev.\unlock()$
			\State $\curr.\unlock()$
			\State \tbf{return} $\result$
			\Statex
		\end{algorithmic}
}


\newcommand{\RemoveGhostFig}{
	\begin{minipage}[c]{4.3cm}
		\RemoveGhostBody
		\label{fig:remove:ghost}
  \end{minipage}
}



\begin{SaveVerbatim}{skiplist-data}
class Skiplist {
	Node* head;
	Node* tail;
	int maxLevel;

}
\end{SaveVerbatim}

\begin{SaveVerbatim}{skiplist-node-data}
class Node {
	Value v;
	Key k;
	Array<Node*>(4) next;
}
\end{SaveVerbatim}



==> figs/ipe/latex/theories.tex <==
%
% T_{fSeq} to T_{path} Auxiliary Functions
%
\newcommand{\TPathFig}{
\renewcommand{\arraystretch}{1}
\centering
\begin{tabular}{|c|}
\hline
$\fApp : \sSeq \times \sSeq \to \sSeq$ \\
\hline
$\fApp (\fNil, l) = l$ \\
$\fApp(\fCons(a,l), l') = \fCons(a, \fApp(l, l'))$ \\
\hline
\hline
$\fSeqToSet : \sSeq \to \sSet$ \\
\hline
$\fSeqToSet (\fNil) = \emptyset$ \\
$\fSeqToSet (\fCons(a,l)) = \{ a \} \cup \fSeqToSet(l)$ \\
\hline
\hline
$\fIsPath : \sSeq$ \\
\hline
$\fIsPath(\fNil)$ \\
$\fIsPath(\fCons(a, \fNil))$ \\
$\{a\} \nsubseteq \fSeqToSet(l) \land \fIsPath(l) \Impl
	\fIsPath(\fCons(a,l))$ \\
\hline
\hline
$\fLast : \sSeq \to \sAddr$ \\
\hline
$\fLast(\fCons(a, \fNil)) = a$ \\
$l \neq \fNil \Impl \fLast(\fCons(a, l)) = \fLast(l)$ \\
\hline
\hline
$\pIsReachK : \sMem \times \sAddr \times \sAddr \times \sLevelK$ \\
\hline
$\pIsReachK(m, a, a, l)$ \\
$m[a].\fNext[l] = a' \land \pIsReach(m, a', b, l)
	\Impl \pIsReach(m, a, b, l)$ \\
\hline
\hline
$\pIsReachKP : \sMem \times \sAddr \times \sAddr \times \sLevelK
	\times \sSeq$ \\
\hline
$\pIsReachKP(m, a, a, l, \fNil)$ \\
$m[a].\fNext[l] = a' \land \pIsReachP(m, a', b, l, p) \Impl
	\pIsReachP(m, a, b, l, \fCons(a, p))$ \\
\hline
\hline
$\fFirstMarked : \sMem \times \sSeq \times \sLevelK \times \sAddr$ \\
\hline
$\fFirstMarked (m, \fNil, l, \fNull)$ \\
$p \neq \fNil \land p = \fCons(j, q) \land m[j].\fLockID[l] \neq \oslash
	\Impl \fFirstMarked(m, p, l, j)$ \\
$p \neq \fNil \land p = \fCons(j, q) \land m[j].\fLockID[l] = \oslash
	\land \fFirstMarked(m, q, l, i)
		\Impl \fFirstMarked(m, p, l, i)$ \\
\hline
\hline
$\pOrdPath : \sMem \times \sSeq$ \\
\hline
$\pOrdPath(h, \fNil)$ \\
$h[a].\fNext[\fLevel{0}] = a' \land h[a].\fKey \pOrd h[a'].\fKey \land
	p = \fCons(a, q) \land \pOrdPath(h, q) \Impl \pOrdPath(h, p)$ \\
\hline
\end{tabular}
}


%
% TLLpL Auxiliary Functions
%
\newcommand{\AuxiliaryFunctions}{
\centering
\begin{tabular}{|c|}
\hline
$\List : \sMem \times \sAddr \times \sSet$ \\
\hline
$\begin{array}{lcl}
	\List(h,a,r) & \Iff & \fNull \in \fAddrToSet(h, a)
		\land r = \fPathToSet(\fGetp(h, a, \fNull)) \\
\end{array}$\\
\hline
\hline
$\fa : \sMem \times \sAddr \to \sPath$ \\
\hline
$\fa(h,n) = \begin{cases}
		\fEpsilon & \trm{if } n = \fNull \\
		\fGetp(h, h[n].\fNext, \fNull) & \trm{if } n \neq \fNull \\
		\end{cases}$ \\
\hline
%
% Begin: Function removed to reduce space
%
%\hline
%$\fb : \sMem \times \sAddr \times \sAddr \times \sPath$ \\
%\hline
%$\begin{array}{lcl}
%\fb(h, n, m, p) & \Iff & (n = \fNull \land p = \fEpsilon)
%	\lor \; \big(n \neq \fNull \land \pReach(h,n,m,\tilde{p})\\
%		&& \hs{3.5} \land \; m = \fNull
%			\Impl \pAppend(p, \fNull, \tilde{p}) \\
%		&& \hs{3.5} \land \; m \neq \fNull
%			\Impl \pAppend(p, [m], \tilde{p}) \big) \\
%\end{array}$ \\
%\hline
\hline
$\LastMarked : \sMem \times \sPath \to \sAddr$ \\
\hline
$\LastMarked(m, p) = \fFirstLocked(m, \fRev(p))$ \\
\hline
\hline
$\NoMarks : \sMem \times \sPath$ \\
\hline
$\NoMarks(m,p) \Iff \fFirstLocked(m,p) = \fNull$ \\
\hline
\hline
$\SomeMark : \sMem \times \sPath$ \\
\hline
$\SomeMark(m,p) \Iff \fFirstLocked(m,p) \neq \fNull$ \\
\hline
\end{tabular}
}



%
% TSLK Signature
%
\newcommand{\TSLKSignature}{
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Signature & \hs{0.1} Sorts \hs{0.1} & Functions & Predicates \\
\hline
\hline
\sigLevelK &
	$\begin{array}{c}
		\sLevelK
	\end{array}$ &
	$\begin{array}{lcl}
		0,1, \ldots, \K-1 & : & \sLevelK \\
	\end{array}$ &
	$\begin{array}{lcl}
		< : \sLevelK \times \sLevelK
	\end{array}$\\
\hline
\sigOrd &
	$\begin{array}{c}
		\sOrd
	\end{array}$ &
	$\begin{array}{lcl}
		\fZero & : & \sOrd \\
		\fInfty & : & \sOrd \\
	\end{array}$ &
	$\begin{array}{lcl}
		\pOrd & : & \sOrd \times \sOrd \\
	\end{array}$ \\
\hline
\sigThId &
	$\begin{array}{c}
		\sThId
	\end{array}$ &
	$\begin{array}{lcl}
		\oslash & : & \sThId \\
	\end{array}$ & \\
\hline
\hline
\sigCells &
	$\begin{array}{c}
		\sCell \\ \sElem \\ \sOrd \\ \sAddr \\ \sThId
	\end{array}$ &
	$\begin{array}{lcl}
		\fError & : & \sCell \\
		\fMkcell & : & \sElem \times \sOrd \times \sAddr^{\K}
			\times \sThId^{\K} \to \sCell \\
		\_.\fData & : & \sCell \to \sElem \\
		\_.\fKey & : & \sCell \to \sOrd \\
		\_.\fNext \lbrack \_ \rbrack & : & \sCell \times \sLevelK
			\to \sAddr \\
		\_.\fLockID \lbrack \_ \rbrack & : & \sCell
			\times \sLevelK \to \sThId \\
		\_.\fLock \lbrack \_ \rbrack & : & \sCell \times \sLevelK	
			\to \sThId \to \sCell \\
		\_.\fUnlock \lbrack \_ \rbrack & : & \sCell
			\times \sLevelK \to \sCell \\
	\end{array}$ & \\
\hline
\sigMemory &
	$\begin{array}{c}
		\sMem \\ \sAddr \\ \sCell
	\end{array}$ &
	$\begin{array}{lcl}
		\fNull & : & \sAddr \\
		\_[\_] & : & \sMem \times \sAddr \to \sCell \\
		\fUpd & : & \sMem \times \sAddr \times \sCell \to \sMem
	\end{array}$ & \\
\hline
\sigReach &
	$\begin{array}{c}
		\sMem \\ \sAddr \\ \sPath
	\end{array}$ &
	$\begin{array}{lcl}
		\fEpsilon & : & \sPath \\
		\lbrack \_ \rbrack & : & \sAddr \to \sPath
	\end{array}$ &
	$\begin{array}{lcl}
		\pAppend & : & \sPath \times \sPath \times \sPath \\
		\pReachK & : & \sMem \times \sAddr \times \sAddr \\
				&& \mhs \times \; \sLevelK \times \sPath \\
	\end{array}$ \\
\hline
\hline
\sigSets &
	$\begin{array}{c}
		\sAddr \\ \sSet
	\end{array}$ &
	$\begin{array}{lcl}
		\emptyset & : & \sSet \\
		\{ \_ \} & : & \sAddr \to \sSet \\
		\cup, \cap, \setminus & : & \sSet \times \sSet \to \sSet
	\end{array}$ &
	$\begin{array}{lcl}
		\in & : & \sAddr \times \sSet \\
		\subseteq & : & \sSet \times \sSet
	\end{array}$ \\
\hline
\sigSetsT &
	$\begin{array}{c}
		\sThId \\ \sSetT
	\end{array}$ &
	$\begin{array}{lcl}
		\stEmpty & : & \sSetT \\
		\stSingle{\_} & : & \sThId \to \sSetT \\
		\stCup, \stCap, \stSubst & : & \sSetT \times \sSetT \to \sSetT
	\end{array}$ &
	$\begin{array}{lcl}
		\stIn & : & \sThId \times \sSetT \\
		\stSubset & : & \sSetT \times \sSetT
	\end{array}$ \\
\hline
\sigMrgn &
	$\begin{array}{c}
		\sMrgn, \\ \sAddr \\ \sLevelK
	\end{array}$ &
	$\begin{array}{lcl}
		\mrgnEmpty & : & \sMrgn \\
		\mrgnSingle{\_, \_} & : & \sAddr \times \sLevelK \to \sMrgn \\
		\mrgnCup, \mrgnCap, \mrgnMinus & : & \sMrgn \times \sMrgn
			\to \sMrgn
	\end{array}$ &
	$\begin{array}{lcl}
		\mrgnIn & : & \sAddr \times \sLevelK \times \sMrgn \\
		\mrgnSubset & : & \sMrgn \times \sMrgn \\
		\mrgnDisj & : & \sMrgn \times \sMrgn
	\end{array}$ \\
\hline
\hline
\sigBridge &
	$\begin{array}{c}
		\sMem \\ \sAddr \\ \sSet \\ \sPath
	\end{array}$ &
	$\begin{array}{lcl}
		\fPathToSet & : & \sPath \to \sSet \\
		\fAddrToSetK & : & \sMem \times \sAddr \times \sLevelK
			\to \sSet \\
		\fGetpK & : & \sMem \times \sAddr \times \sAddr \times
			\sLevelK \to \sPath \\
		\fFirstLockedK & : & \sMem \times \sPath \times \sLevelK
			\to \sAddr
	\end{array}$ &
	$\begin{array}{lcl}
		\pOrdList & : & \sMem \times \sPath \\
	\end{array}$ \\
\hline
\end{tabular}
}


%
% TSLK Interpretations
%
\newcommand{\TSLKInterpretationsOne}{
\centering
\begin{tabular}{|c|p{10.5cm}|}
\hline
\multicolumn{2}{|c|}{Interpretation of sort symbols: \sAddr, \sElem, 
\sThId, \sLevelK, \sOrd, \sCell, \sMem, \sPath, \sSet, \sSetT and \sMrgn}
\\
\hline
\hline
\multicolumn{2}{|l|}{
Each sort $\sigma$ in \sigTSLK is mapped to a non-empty set $\Ais{\sigma}$ 
such that:} \\
\multicolumn{2}{|l|}{
\begin{tabular}{clcl}
	(a) &$\Ais{\sAddr}$ and $\Ais{\sElem}$ are discrete sets &
	(b) &$\Ais{\sThId}$ is a discrete set containing symbol $\oslash$ \\
	(c) &$\Ais{\sLevelK}$ is the finite collection 0,\ldots,\K-1 &
	(d) &$\Ais{\sOrd}$ is a collection of total ordered identifiers \\
	(e) &$\Ais{\sCell} = \Ais{\sElem} \times \Ais{\sOrd} \times 
		\Ais{\sAddr}^{\K} \times \Ais{\sThId}^{\K}$ &
	(f) &$\Ais{\sMem} = \Ais{\sCell}^{\Ais{\sAddr}}$ \\
	(g) &$\Ais{\sPath}$ is the set of all finite sequences of &
	(h) &$\Ais{\sSet}$ is the power-set of $\Ais{\sAddr}$ \\
		& \hs{0.5} (pairwise) distinct elements of $\Ais{\sAddr}$ &
	(i) &$\Ais{\sSetT}$ is the power-set of $\Ais{\sThId}$ \\
	(j) &$\Ais{\sMrgn}$ is the power-set of
		$\Ais{\sAddr} \times \Ais{\sLevelK}$ &
\end{tabular}
} \\
\hline
\hline
Signature & Interpretation \\
\hline
%\hline
%\sigLevelK &
%	\begin{tabular}{p{9.7cm}}
%		$\inter{\fLevel{i}}{\Ai} \neq \inter{\fLevel{j}}{\Ai}$
%			when $i \neq j$
%	\end{tabular} \\
\hline
\sigOrd &
	\begin{tabular}{p{9.7cm}}
		$x \inter{\pOrd}{\Ai} y \land y \inter{\pOrd}{\Ai} x
			\Impl x = y$ for any $x, y \in \Ais{\sOrd}$ \\
		$x \inter{\pOrd}{\Ai} y \land y \inter{\pOrd}{\Ai} z
			\Impl x \inter{\pOrd}{\Ai} z$
			for any $x, y, z \in \Ais{\sOrd}$ \\
		$x \inter{\pOrd}{\Ai} y \lor y \inter{\pOrd}{\Ai} x$
			for any $x, y \in \Ais{\sOrd}$ \\
		$\inter{\fZero}{\Ai} \inter{\pOrd}{\Ai} x \land
		x \inter{\pOrd}{\Ai} \inter{\fInfty}{\Ai}$
			for any $x \in \Ais{\sOrd}$ \\
%		$x \neq \inter{\fInfty}{\Ai} \Impl
%			x \inter{\pOrd}{\Ai} \inter{\fSucc}{\Ai}(x)$
%			for any $x \in \Ais{\sOrd}$ \\
	\end{tabular} \\
\hline
\hline
\sigCells &
	\begin{tabular}{p{11.5cm}}
		\begin{compactitem}
		\item $\inter{\fMkcell}{\Ai} (e, k, a_0, \ldots, a_{\K-1},
						t_0, \ldots, t_{\K-1}) =
			\langle e, k, a_0, \ldots, a_{\K-1},
				t_0, \ldots, t_{\K-1} \rangle$
			for each
			$e \in \Ais{\sElem}$, $i \in \Ais{\sOrd}$,
			$a_0, \ldots, a_{\K-1} \in \Ais{\sAddr}$
			and $t_0, \ldots, t_{\K-1} \in \Ais{\sThId}$
		\item $\langle e, k, \vect{a}, \vect{t} \rangle
				.\inter{\fData}{\Ai} = e$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$
			and $\vect{t} \in \Ais{\sThId}^{\K}$
		\item $\langle e, k, \vect{a}, \vect{t} \rangle
				.\inter{\fKey}{\Ai} = k$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$
			and $\vect{t} \in \Ais{\sThId}^{\K}$
		\item $\langle e, k, a_0, \ldots, a_{\K-1}, \vect{t} \rangle
				.\inter{\fNext}{\Ai}[j] = a_j$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$a_0 \ldots, a_{\K-1} \in \Ais{\sAddr}$,
			$j \in \Ais{\sLevelK}$
			and $\vect{t} \in \Ais{\sThId}^{\K}$ and
		\item $\langle e, k, \vect{a}, t_0, \ldots, t_{\K-1} \rangle
				.\inter{\fLockID}{\Ai}[j] = t_{j}$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$,
			$j \in \Ais{\sLevelK}$
			and $t_0, \dots, t_{\K-1} \in \Ais{\sThId}$
		\item $\langle e, k, \vect{a}, t_0, \ldots, t_{\K-1} \rangle
				.\inter{\fLock}{\Ai}[j](t') =
			\langle e, k, \vect{a},
				t_0, \ldots, t_{j-1}, t',
				t_{j+1}, \ldots, t_{\K-1}
			\rangle$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$,
			$j \in \Ais{\sLevelK}$
			and $t_0, \ldots, t_{\K-1}, t' \in \Ais{\sThId}$
		\item $\langle e, k, \vect{a}, t_0, \ldots, t_{\K-1} \rangle
				.\inter{\fUnlock}{\Ai}[j] =
			\langle e, k, \vect{a},
				t_0, \ldots, t_{j-1}, \oslash,
				t_{j+1}, \ldots, t_{\K-1}
			\rangle$
			for each $e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$,
			$j \in \Ais{\sLevelK}$
			and $t_0, \ldots, t_{\K-1} \in \Ais{\sThId}$
		\item $\inter{\fError}{\Ai}.\inter{\fNext}{\Ai} =
			\inter{\fNull}{\Ai}$
		\end{compactitem}
	\end{tabular} \\
\hline
\sigMemory &
	\begin{tabular}{p{9.7cm}}
		\begin{compactitem}
		\item $m\inter{[a]}{\Ai} = m(a)$ for each $m \in \Ais{\sMem}$
			and $a \in \Ais{\sAddr}$
		\item $\inter{\fUpd}{\Ai}(m,a,c) = m_{a \mapsto c}$ for each
			$m \in \Ais{\sMem}$, $a \in \Ais{\sAddr}$ and
			$c \in \Ais{\sCell}$
		\item $\inter{m}{\Ai}(\inter{\fNull}{\Ai}) = 
			\inter{\fError}{\Ai}$
			for each $m \in \Ais{\sMem}$
		\end{compactitem}
	\end{tabular} \\
\hline
\sigReach &
	\begin{tabular}{p{11cm}}
		\begin{compactitem}
		\item $\inter{\fEpsilon}{\Ai}$ is the empty sequence
		\item $\inter{[i]}{\Ai}$ is the sequence containing $i \in 
			\Ais{\sAddr}$ as the only element
		\item $\left(\left[i_1,\ldots, i_n\right], \left[j_1, \ldots, 
			j_m\right], \left[i_1,\ldots, i_n, j_1,
				\ldots, j_m\right]
			\right) \in \inter{\pAppend}{\Ai}$ iff $i_k$
		and $j_l$ are all distinct
		\item $(m, \aInit, \aEnd, l, p) \in \inter{\pReachK}{\Ai}$
			iff $\aInit=\aEnd$ and $p = \fEpsilon$, or
		there exist addresses $a_1, \ldots, a_n \in \Ais{\sAddr}$ such 
		that:
		\end{compactitem} \\
		\hs{1.5} $\begin{array}{ll}
			\trm{(a) } p = [a_1, \ldots, a_n]  \phantom{aaaa}&
			\trm{(c) } m(a_r).\inter{\fNext}{\Ai}[l]
				= a_{r+1}, \trm{for } 1 \leq r < n \\
			\trm{(b) } a_1 = \aInit &
			\trm{(d) } m(a_n).\inter{\fNext}{\Ai}[l]
				= \aEnd
		\end{array}$
	\end{tabular} \\
\hline
\hline
\sigSets &
	\begin{tabular}{p{11cm}}
		The symbols $\emptyset$, $\{ \_ \}$, $\cup$, $\cap$, 
		$\setminus$, $\in$ and $\subseteq$ are interpreted 
according to
		their standard interpretation over sets of addresses.
	\end{tabular} \\
\hline
\sigSetsT &
	\begin{tabular}{p{11cm}}
		The symbols $\stEmpty$, $\stSingle{\_}$, $\stCup$, $\stCap$, 
		$\stSubst$, $\stIn$ and $\stSubset$ are interpreted according
		to their standard interpretation over sets of thread
		identifiers.
	\end{tabular} \\
\hline
\end{tabular}
}


\newcommand{\TSLKInterpretationsTwo}{
\centering
\begin{tabular}{|c|p{11.7cm}|}
\hline
Signature & Interpretation \\
\hline
\hline
\sigMrgn &
	\begin{tabular}{p{11cm}}
		\begin{compactitem}
		\item $\mrgnEmptyI{\Ai} = \emptyset$
		\item $\mrgnSingleI{a,j}{\Ai} = \{ (a,j) \}$
			for each $a \in \Ais{\sAddr}$
			and $j \in \Ais{\sLevelK}$
		\item $m_1 \mrgnCupI{\Ai} m_2 = m_1 \cup m_2$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\item $m_1 \mrgnCapI{\Ai} m_2 = m_1 \cap m_2$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\item $m_1 \mrgnMinusI{\Ai} m_2 = m_1 \setminus m_2$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\item $m_1 \mrgnSubsetI{\Ai} m_2 \Iff m_1 \subseteq m_2$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\item $(a,j) \mrgnInI{\Ai} m \Iff (a,j) \in m$
			for each $a \in \Ais{\sAddr}$,
			$j \in \Ais{\sLevelK}$ and $m \in \Ais{\sMrgn}$
		\item $m_1 \mrgnDisjI{\Ai} m_2 \Iff m_1 \mrgnCapI{\Ai} m_2
			= \mrgnEmptyI{\Ai}$
			for each $m_1, m_2 \in \Ais{\sMrgn}$
		\end{compactitem}
	\end{tabular} \\
\hline
\hline
\sigBridge &
	\begin{tabular}{p{11cm}}
		\begin{compactitem}
		\item $\inter{\fPathToSet}{\Ai}(p) = \{ a_1, \ldots, 
			a_n\}$ for $p = [a_1, \ldots, a_n] \in
			\Ais{\sPath}$
		\item $\inter{\fAddrToSetK}{\Ai}(m, a, l) = \big\{
			a' \in \Ais{\sAddr} \:|\: \exists p \in 
			\Ais{\sPath}$ s.t. $(m,a,a',l,p) \in \pReachK
			\big\}$
		\item $\inter{\fGetpK}{\Ai}(m,\aInit,\aEnd,l) =
			\begin{cases}
				p & \text{if } (m,\aInit,\aEnd,l,p)
					\in \inter{\pReachK}{\Ai} \\
				\fEpsilon & \text{otherwise}
			\end{cases}$
		\end{compactitem} \\
			\hspace{1cm} for each $m \in \Ais{\sMem}$,
			$p \in \Ais{\sPath}$, $l \in \Ais{\sLevelK}$
			and $\aInit, \aEnd \in \Ais{\sAddr}$
		\begin{compactitem}
		\item $\inter{\fFirstLocked}{\Ai}\left(m,[a_1, \ldots,
			a_n], l \right) =\left\{
			\begin{array}{ll}
			a_k &
			\trm{if there is } 1 \leq k \leq n \trm{ such that } \\
			& \trm{for all } 1 \leq j < k,
				m[a_j].\fLockID[l] = \oslash \\
			& \trm{and } m[a_k].\fLockID[l] \neq \oslash \\
			\fNull & \trm{otherwise }
			\end{array}
			\right.$
		\item $\inter{\pOrdList}{\Ai}\left(m,p \right)$
			iff $p=\fEpsilon$ or $p = \lbrack a \rbrack$ or
			$p = [a_1, \ldots, a_n]$ with $n \geq 2$ and
			$m(a_i).\inter{\key}{\Ai} \pOrd
				m(a_{i+1}).\inter{\key}{\Ai}$
			for all $1 \leq i < n$,
			for any $m \in \Ais{\sMem}$
		\end{compactitem}
	\end{tabular} \\
\hline
\end{tabular}
}


==> figs/ipe/latex/vpl-macros.tex <==
\newcommand{\val}[1]{\ensuremath{[\![ #1 ]\!]}}
\newcommand{\der}[1]{\ensuremath{{\mathop{{ %
            \longrightarrow}}\limits^{{#1}}}\!}} %
\newcommand \tpl[1]{\langle #1 \rangle}
%\newcommand{\RE}{\textsf{RE}\xspace}
\newcommand{\NVPA}{\textsf{NVPA}\xspace}
\newcommand{\VPA}{\textsf{VPA}\xspace}
\newcommand{\NFA}{\textsf{NFA}\xspace}
\newcommand{\VPL}{\textsf{VPL}\xspace}
\newcommand{\CARET}{\textsf{CaRet}\xspace}
\newcommand{\VPLs}{\textsf{VPL}s\xspace}
\newcommand{\VRL}{\textsf{VRL}\xspace}
\newcommand{\VRE}{\textsf{VRE}\xspace}
\newcommand{\EMSO}{\textsf{MSO$_{\mu}$}\xspace}
\newcommand{\MSO}{\textsf{MSO}\xspace}
\newcommand{\XML}{\textsf{XML}\xspace}

\newcommand{\EXPTIME}{{\sffamily EXPTIME}\xspace}

\newcommand{\WM}{\ensuremath{\mathit{WM}}\xspace}
\newcommand{\MR}{\ensuremath{\mathit{MR}}\xspace}
\newcommand{\MC}{\ensuremath{\mathit{MC}}\xspace}
\newcommand{\SWM}{\ensuremath{\mathit{MWM}}\xspace}
\newcommand{\Pu}{\ensuremath{\mathcal{P}}\xspace}
%\newcommand{\Lang}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\Au}{\ensuremath{\mathcal{A}}}
\newcommand{\Msubst}{$M$-substitution\xspace}
\newcommand{\Mclosure}{$M$-closure\xspace}
\newcommand{\Sclosure}{$S$-closure\xspace}


\newcommand{\Stilde}{\widetilde{\Sigma}\xspace}
\newcommand{\Scall}{\Sigma_{\mathit{call}}\xspace}
\newcommand{\Sret}{\Sigma_{\mathit{ret}}\xspace}
\newcommand{\Sint}{\Sigma_{\mathit{int}}\xspace}

\newcommand{\SubstOp}[1]{\mathrel{\curvearrowleft_{#1}}}
\newcommand{\SubstBox}{\SubstOp{\Box}}
\newcommand{\MClos}[2]{#1^{\SubstOp{#2}}}
\newcommand{\LangClos}{\MClos{\Lang}{\Box}}
\newcommand{\SClos}[2]{{#1}^{\circlearrowleft_{#2}}}
\newcommand{\SClosure}[1]{\SClos{#1}{\Box}}
\newcommand{\LangSClos}{\SClos{\Lang}{\Box}}



%\newcommand{\DefinedAs}{\,\stackrel{\text{def}}{=}\,}

%\newcommand{\DefOR}{\ensuremath{\;\;\;\big|\;\;\;}}
\newcommand{\DefORmini}{\ensuremath{\;\;\big|\;\;}}

\newcommand{\details}[1]{}

\newcommand{\Outcm}{c\,b\,r}
\newcommand{\UOutcm}{\underline{\Outcm}}

\newcommand{\LSet}{R}
\newcommand{\SSet}{S}

\newcommand{\qin}{\ensuremath{q_{\textit{in}}}}

==> ideas.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage
%\section{Categories}
%
%\begin{table}[h!]
%		\renewcommand{\arraystretch}{1.2}	 
%		\begin{tabular}{|| l || l |  l || }
%			\hline
%				 		& $\Box \varphi$ & $\F \varphi$ \\
% \hline		
%$\forall \msmall$  $\exists \mbig$ 
%& \thead[l]{\regs \\
%	\tabitem Certificate Translation (Matrix Multi) \\
%	\tabitem Scenario Programming (ABP Protocol)}
%& \thead[l]{\unroll \\ 
%	\tabitem 1 \\
%	\tabitem 2} \\
%\hline
%$\forall \mbig$  $\exists \msmall$ 
%& \thead[l]{\regs \\
%	\tabitem \\ 
%	\tabitem} 
%& \thead[l]{\unroll \\ 
%	\tabitem 1 \\
%	\tabitem 2}\\
%\hline \hline
%$\exists \msmall$  $\forall \mbig$ 
%& \thead[l]{\eas \\
%	\tabitem \\  
%	\tabitem} 
%& \thead[l]{\unroll \\ 
%	\tabitem 1 \\
%	\tabitem 2}\\
%\hline
%$\exists \mbig$  $\forall \msmall$ 
%& \thead[l]{\eas \\
%	\tabitem \\
%	\tabitem}
%& \thead[l]{\unroll \\
%	\tabitem 1 \\
%	\tabitem 2} \\
%		\end{tabular}	
%\end{table}
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section{Ideas for Case Studies}


\noindent{$\forall \pi [M_1: small].\  \exists \pi' [M_2: large].$   {\it Box property always holds if \regs\ exists.}}



\begin{itemize}
%%%
\item {\bf Scenario programming (behavioral programming)}\\ 
Abstract design  are in message sequence chart (MSC) and live sequence chart (LSC). The goal is to synthesize the desired program, and further test it using verification tools. 
	\begin{itemize}[label={$\circ$}]
		\item ~{\color{blue} [HVC’14]:
		Synthesis ABP protocol with 4 scenarios (example behaviors) and a set of temporal specification(safety/liveness)}. 
%		\item ~[TACAS’05]: existential and universal behaviors. 
%		\item ~[FM’05] 
%		\item ~[Conext'15]:
	\end{itemize}


%%%
\item {\bf Certificate translation}  \\
Source + (proof, advice, certificate,…) to  Target + (proof’, advice’, certificate’,…). Translate proof to proof’ to guarantee the correctness of the target program to deal with untrusted intermediaries such as compiler, translator, etc.
\begin{itemize}[label={$\circ$}] 
	\item ~ {\color{blue} [Barthe'09] Matrix Multiplication program, from
		high-level code (C) $\rightarrow$ property (ACSL) $\rightarrow$ low-level code (RTL)} 
\end{itemize}

%%%
\item {\bf Programming by Example (PBE)} 
	\begin{itemize}[label={$\circ$}]
	\item ~[vldb'18]: Use code-by-example to form a program that transforms `Hierarchical data models` to `relational format` 
	\item ~[untrustedCG]: 
	\end{itemize}
	
%%%	
\item {\bf Composability of interface automatas} \\
For automatic compatibility check. (Checking the interfaces of two components are compatible. It is computing `two interfaces` instead of with the implementation.
	\begin{itemize}[label={$\circ$}]
	\item ~[Henzinger'01]
	\end{itemize}

\item {\bf Sequentialization} \\
Synthesize and verify the sequentialization of some concurrent programs. Sequential program over-approximates the semantics of the  original distributed program, safety properties are thus proved. (They are always ‘equivalent’)



%%%
%\item {\bf Secure Hardware Design}  \\
%Register Transfer Level Informatino Flow Tracking (RTIFT). 
%	\begin{itemize}[label={$\circ$}] 
	%	\item ~[DATE'17] 
	%	\end{itemize}

%%%
\item {\bf Verifying compiled programs (secure compilation)}\\
Verifying source and target programs compiled by a compiler.
Cannot locate on papers that provide concrete examples of before/after compilation, except for the optimization paper.
\begin{itemize}[label={$\circ$}]
	\item ~[optimization paper]
\end{itemize}
%				\textcolor{red}{cannot locate on papers that provide concrete examples of before/after compilation, except for the [optimization paper]}


%%%
\item {\bf Behavioral conformance} 

%%%
\item \underline{Model/Program transformation verification (M2M)}

%%%
\item \underline{Flows}
\end{itemize}

%\noindent{$\exists \pi [M_1: large]. \forall \pi' [M_2: small].\ $   {\it Box property always holds if \eas\  exists.}}



==> logs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section{Meeting Notes}


\subsection{(Initial Idea) Finite Enumeration of Loops}
Explore each simple loops of the forall quantifier in $\forall\exists$ formula.

\begin{algorithm}
	\caption{Matching Simple Loops}\label{alg:cap}
		for each $\ell$ in loops of $\forall$ model: \\
		~~~increase bound $k$ \\
		~~~find $\ell'$ in $\exists$ model that matches $\ell$\\
		~~~return when each $\ell$ in the $\forall$ model has a matching $\ell'$ in $\exists$ model.
\end{algorithm}




\subsection{Models as Language}
Decompose $\forall$ model as language $L(M_A)$, which can be 
decomposed into:
$$|\{ L_1 \cup L_2 \cup L_2 \cup \ldots \cup L_m \}| \geq  |L(M_A)|$$
Each $L_i$ must have {\em some properties} (i.e., simple candidates)

$$M = \langle M_1, M_2, \ldots, M_m \rangle, M \models \varphi \text{  iff  }  
 \langle C_1, C_2, \ldots, C_m \rangle \models \varphi$$

The number of lasso paths is bounded by the size of automaton, so it limits the search. 


\newcommand{\invi}{{invisible}}
\newcommand{\visi}{{visible}}
\subsection{Visible and Invisible States}
Over-/Under-approximation by classifying some states as `invisible` (i.e., sink, or don't-care states). The transition relation $R(x, x')$ becomes:

$$ ( \invi_x \rightarrow \invi_{x'}) \land (\visi_x \rightarrow R(x, x'))  $$
 

\subsection{Simulations}
\begin{itemize}
	\item Full-exploration for $\forall$ and under-approximation for $\exists$	
	\item Over-approximation for $\forall$ and under-approximation for $\exists$
	\item IC3? (for loops)
\end{itemize}

\noindent QBF Encoding for simulations.

\noindent SAT Encoding  for simulations.

\vspace{3mm}
\noindent{\bf Fair Simulation}

Fairness constraints$F$ that decides a fair-run. 
\begin{itemize}
	\item weak (Buchi) fair
	\item strong (Streett) fair
\end{itemize}
 $M_2$ fair simulate $M_1$ if all fair-run in $M_1$ has a matching fair-run in $M_2$.


\vspace{3mm}
\noindent{\bf Tasks:}
\begin{enumerate}
	\item Make $\forall \exists$ simulation complete (for $\forall \exists \G \varphi$).
	\item Formalize $\exists \forall \G \varphi$ algorithm.
	\item Explore abstractions.
\end{enumerate}


\vspace{3mm}
\noindent{\bf Bounded Prophecy in Simulation}

If some branches are far from the initial states, it is possible that $\forall\exists$ simulation is not available but $\langle M_1, M_2 \rangle \models \G \varphi$\\

\noindent {\question Q: enumerating prophecy?}\\
\noindent {\question Q: sophisticated prophecy?}


\vspace{3mm}
\noindent{\bf Completeness}

Run two algorithms with incremental search (simulation with bound $k$, and unrolling with bound $k$) and eventually  one of them will halt.\\

\includegraphics[scale=.2]{table}

\subsection{Good Abstraction (from Cesar's note)}
We can find $\exists\forall \G \varphi$ more efficiently by selecting a good abstraction for the second model. For example, consider 
$$
\varphi = \G(\neg p_{\pi_1} \lor \neg p_{\pi_2})
$$
Then the `worst choice` for $M_2$ is $p^\omega$. That is, for every $a'_0, a'_1, a'_2, \ldots \in L_{M'_2}$, there is $a_0, a_1, a_2, \ldots \in L_{M_2}$, such that $a'_0 \models \neg p$ then $a_0 \models \neg p$.





==> related.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
\label{sec:related}

Hyperproperties was first introduced by Clarkson and Schneider~\cite{cs10}, and the first algorithms for model checking HyperLTL and HyperCTL$^*$ were introduced in~\cite{frs15}, which was using alternating automata.
%
Automated reasoning about \hltl specifications has been getting a lot of progress 
in many aspects
including verifying~\cite{frs15,fmsz17,fht18,cfst19} and monitoring~\cite{ab16,fhst19,bsb17,bss18,fhst18,sssb19,hst19}.
%
With this growing amount of research, many tools can also support \hltl, 
including \code{MCHyper}~\cite{frs15,cfst19} for model checking, 
\code{EAHyper}~\cite{fhs17} and \code{MGHyper}~\cite{fhh18} for satisfiability checking, 
and \code{RVHyper}~\cite{fhst18} for runtime monitoring.
%
However, the aforementioned tools are limited to \hltl formulas without quantifier alternations. 
%
Recently, this difficulty of alternating formulas was tackled by the bounded  model 
checker \code{HyperQube}~\cite{hsu21bounded} using QBF solving.
%
However, \code{HyperQube} is lack of practical loop conditions that allows to 
capture early infinite traces in finite exploration.
%
In this paper, we develop the simulation-based algorithm to resolve it.
%
Furthermore, while there are more than one approach to reason about infinite traces, 
another line of work applies {\em strategy-based} approach 
to deal with formulas in the form of $\forall\exists$~\cite{coenen19verifying}, and the incompleteness can be resolved by generating 
a set of prophecy variables~\cite{beutner2022prophecy}.
% 
However, in this work we capture infinity 
in a more efficient manner using simulation.
%
We also build an applicable prototype for reasoning
\hltl formulas with models that contain loops.  




 


%
%There has been a lot of recent progress in automatically
%verifying~\cite{frs15,fmsz17,fht18,cfst19} and
%monitoring~\cite{ab16,fhst19,bsb17,bss18,fhst18,sssb19,hst19} HyperLTL
%specifications.
%%
%HyperLTL is also supported by a growing set of tools, including the
%model checker \code{MCHyper}~\cite{frs15,cfst19}, the satisfiability checkers
%\code{EAHyper}~\cite{fhs17} and \code{MGHyper}~\cite{fhh18}, and the runtime
%monitoring tool \code{RVHyper}~\cite{fhst18}.
%%
%The complexity of \emph{model checking} for HyperLTL for
%tree-shaped, acyclic, and general graphs was rigorously investigated
%in~\cite{bf18}.
%%
%The first algorithms for model checking HyperLTL and HyperCTL$^*$
%using alternating automata were introduced in~\cite{frs15}.
%%
%These techniques, however, were not able to deal in practice with
%alternating HyperLTL formulas in a fully automated fashion.
%%
%We also note that previous approaches that reduce model checking
%HyperLTL---typically of formulas without quantifier alternations---to
%model checking LTL can use BMC in the LTL model checking phase.
%%
%However, this is a different approach than the one presented here, as
%these approaches simply instruct the model checker to use a BMC
%\emph{after} the problem has been fully reduced to an LTL model
%checking problem while we avoid this translation.
%%
%These algorithms were then extended to deal with hyperliveness and
%alternating formulas in~\cite{cfst19} by finding a winning strategy in
%$\forall\exists$ games.
%%
%In this paper, we take an alternative approach by reducing the model
%checking problem to QBF solving, which is arguably more effective for
%finding bugs (in case a finite witness exists).
%
%The {\em satisfiability} problem for HyperLTL is shown to be
%undecidable in general but decidable for the $\exists^*\forall^*$
%fragment and for any fragment that includes a $\forall\exists$
%quantifier alternation~\cite{fh16}.
%%
%The hierarchy of hyperlogics beyond HyperLTL were studied
%in~\cite{cfhh19}.
%%
%The synthesis problem for HyperLTL has been studied
%in~\cite{bf19} in the form of {\em program repair}, in~\cite{bf20} in
%the form of {\em controller synthesis}, and in~\cite{fhlst20} for the
%general case.

==> texs/bmc_npc.tex <==
\subsection{Bounded Simulation}
Let $K_1$ and $K_2$ be two Kripke structures over $AP$, and let $k\in \naturals$. 
The {\em bounded simulation problem} for $K_1,K_2$ and $k$ is to decide whether there exists a simulation relation from $K_1$ to $K_2$ that uses at most $k$ states of $K_2$ (note that in any case, all of the reachable states of $K_1$ must be used in such a simulation). 
We prove this problem to be \comp{NP-complete}.


\begin{theorem}
The bounded simulation problem is \comp{NP-complete}.
\end{theorem}
\begin{proof}
Let $K_1$ and $K_2$ be two Kripke structures with sets of states $Q_1$ and $Q_2$, respectively, and let $k\in \naturals$. 
A nondeterministic algorithm which guesses a set $Q'_2\subseteq Q_2$ of at most $k$ states, and searches for a simulation from $K_1$ to $K_2$ reduced to $Q'_2$. Finding a simulation can be done in polynomial time, and so the problem is in \comp{NP}.

We prove \comp{NP-hardness} by a reduction from the Vertex Cover problem. Given a directed graph $G=\tuple{V,E}$ where $|E|=m$ and where $V=\{v_1,\ldots v_n\}$, and $k\in\naturals$, we construct two Kripke structures $K_1$ and $K_2$, as follows.

$K_1$ is composed of $m$ states, where for every $e\in E$ there is a state labeled $e$, and an additional initial state $q$ labeled $q$. The transitions are from $q$ to all edge states and vice versa. 

$K_2$ is composed of $m$ states similarly labeled as the edge states of $K_1$, and additional $n$ states $v_1,\ldots v_n$  all labeled $q$, all initial. From every $v_i$ there are transitions to all edge states. From every edge state $(v_i,v_j)$ there are transitions to $v_i$ and $v_j$. 

It is easy to see that $K_2$ can simulate $K_1$ using at most $m+k$ states iff $G$ has a vertex cover of size at most $k$.
\end{proof}

Now, let $K_1, K_2$, and $k$ be as before. 
The {\em bounded $\exists\forall$-problem} for $K_1,K_2$ and $k$ is to decide whether there exists a path in $K_1$ which uses at most $k$ states, which is equivalent to all paths in $K_2$. In other words, we ask whether there exists such a path witnessing the hyper-LTL formula $\exists\pi_1\forall\pi_2 \G \bigwedge_{q\in AP}(q_{\pi_1} \iff q_{\pi_2})$.  
We prove this problem to be \comp{NP-complete}.

\begin{theorem}\label{thm:bounded_simulation_NPC}
The bounded $\exists\forall$-problem is \comp{NP-complete}.
\end{theorem}
\begin{proof}

Let $K_1$ and $K_2$ be two Kripke structures with sets of states $Q_1$ and $Q_2$, respectively, and let $k\in \naturals$. 

For the upper bound, we notice that in a yes-instance of the problem, all of the paths in $K_2$ must be equally labeled. This holds iff for every state $s$ in $K_2$, all the transitions from $s$ lead to equally labeled states, a condition which can easily be checked. 

Then, to check that there is a path in $K_1$ that is equal to all paths in $K_2$ which uses at most $k$ states, we can guess $k$ states of $K_1$, and check the nonemptiness of the intersection of $K'_1$ with $K_2$, where $K'_1$ is $K_1$ reduced to the $k$ chosen states. Since intersecting and checking for nonemptiness can be done in polynomial time, we are done. 

We prove \comp{NP-hardness} by a reduction from the Vertex Cover problem. Given a directed graph $G=\tuple{V,E}$ where $|E|=\{e_1,e_2,\ldots e_m\}$ and where $V=\{v_1,\ldots v_n\}$, and $k\in\naturals$, we construct two Kripke structures $K_1$ and $K_2$, as follows.

$K_1$ is $K_2$ of the proof of Theorem~\ref{thm:bounded_simulation_NPC}.  

$K_2$ is composed of $2m$ states $q_1,q_2,\ldots q_{2m}$ arranged in a simple cycle, where $q_1$ is initial. The states in the odd indices are all labeled $q$, and for every $1\leq i\leq m$, state $q_{2i}$ is labeled by $e_i$ .
That is, the cycle enumerates all edges. 

It is easy to see that there exists a path in $K_1$ that uses at most $m+k$ states that is equivalent to (the single) path in $K_2$ iff $G$ has a vertex cover of size at most $k$.

\end{proof}

==> texs/lassos_are_enough.tex <==
Let $M = \tuple{Q,R,I,L}$ be a Kripke Structure over $AP$. A {\em lasso path} of $M$ is a path $q_0,q_1,\ldots,q_k$ such that $q_k = q_i$ for some $1\leq i<k$. This lasso path induces the {\em lasso trace} (or, simply, {\em lasso}) $L(q_0)\dots L(q_{i-1}) (L(q_i)\dots L(q_{k-1}))^\omega$. 

Let $\tuple{M_1,\ldots M_k}$ be a multi-model. We denote the set of lasso traces of $M_i$ by $C_i$. 

\begin{theorem}
Let $M = \tuple{M_1,\ldots M_k}$ be a multi-model, and let $\f = \quant_1 \pi_1\cdots\quant_k \pi_k\g$ be a hyperLTL formula, both over $AP$. 
Then $M\models \f$ iff $\tuple{C_1,\ldots C_k}\models \f$.
\end{theorem}

\begin{proof}
First, we recall the automata-based hyperLTL model-checking procedure of~\cite{}. 
For an LTL formula $\g$ over $AP\times \{\pi_i\}_{i=1}^{k}$, 
we denote  the translation of $\g$ to a B{\"u}chi automaton over $2^{AP\times \{\pi_i\}_{i=1}^{k}}$ by $A_\g$. 

We further define the satisfaction of an automaton $A$ over $2^{AP\times \{\pi_i\}_{i=1}^{k}}$ and a {\em quantification condition} of the type $\alpha = \quant_1 \pi_1\cdots\quant_k \pi_k$ by a multi model $M  =\tuple{M_1,M_2,\ldots M_k}$, as follows.
First, notice that a run of $A$ can be thought of as a joint run of $k$  words $w_1,\ldots w_k$, where $w_i$ is assigned to $\pi_i$. We view this is a run of $A$ on $\tuple{w_1,\ldots w_k}$.

Let $\zeta$ be a function that maps some trace $w_i\in L(M_i)$ to $\pi_i$, for every $1\leq i\leq k$.
We denote $M\models_\zeta \epsilon,A$, if the joint run of $w_1,\ldots, w_k$ is accepted in $A$ (that is, $\tuple{w_1,\ldots w_k}\in L(A)$). 
For $\alpha = \exists_{\pi_1}\alpha'$, we denote $M\models_\zeta \alpha,A$ if there exists $w_1\in L(M_1)$ such that $M\models_{\zeta[\pi_1\mapsto w_1]} \alpha', A$. 
For $\alpha = \forall_{\pi_1}\alpha'$, we denote $M\models_\zeta \alpha,A$ if for every $w_1\in L(M_1)$ it holds that $M\models_{\zeta[\pi_1\mapsto w_1]} \alpha', A$. That is, we define similar semantics to hyperLTL, adjusted to B{\"u}chi automata. As usual, if $A$ is fully quantified by $\alpha$, then satisfaction is independent of $\zeta$ and we denote $M\models \alpha,A$. 


For a B{\"u}chi automaton $A$ over $2^{AP\times \{\pi_i\}_{i=1}^{k}}$ and a model $M$ over $AP$, the automaton  $M\cap_k A$ is the intersection construction for $M$ w.r.t. $AP\times \{x_k\}$, while taking the projection of the result over $AP\times \{\pi_i\}_{i=1}^{k-1}$.
Thus, the language of $M\cap_k A$ is $\{w\in 2^{AP\times \{\pi_i\}_{i=1}^{k-1} } | \exists w'\in L(M_k). w\cup w'_{\pi_k} \in L(A)\}$, where $w\cup w'_{\pi_k}$ denotes the word $w_0\cup \{w'_{0_{\pi_k}}\}\cdot w_1\cup\{w'_{1_{\pi_k}}\}\cdots $. 
Similarly, the language of $M\cap_k \overline{A}$ is $\{w\in 2^{AP\times \{\pi_i\}_{i=1}^{k-1} } | \exists w'\in L(M_k). w\cup w'_{\pi_k} \notin L(A)\}$, and so the language of $\overline{M\cap_k \overline{A}}$ is $\{w\in 2^{AP\times \{\pi_i\}_{i=1}^{k-1} }|\forall w'\in L(M_k). w\cup w'_{\pi_k}\in L(A)\}$.

Given $M$ and $\f$, we construct a sequence $A_k,A_{k-1},\ldots A_2$ of B{\"u}chi automata, as follows.
If $\quant_k = \exists$, then we set $A_k = M_k\cap_k A_\g$. 
Otherwise, $\quant_k = \forall$, and we set 
$A_k = \overline{M_k\cap_k A_{\neg\g}}$.
For every $1< i< k$, if $\quant_i = \exists$ then we set $A_i = M_i\cap_i A_{i+1}$, and if $\quant_i = \forall$ then we set $A_i = \overline{M_i\cap{\overline{A_{i+1}}}}$. 
By the semantics of the quantifiers, for every $1< i \leq k$, it holds that $\tuple{M_1,\ldots, M_i}\models \alpha_i, A_{i+1}$ iff $\tuple{M_1,\ldots, M_k}\models \f$, where $\alpha_i = \quant_1\pi_1\dots \quant_i\pi_i$.

We now proceed to prove that $M\models \f$ iff $\tuple{C_1,\ldots C_k}\models \f$, by induction on $k$.
For $k=1$, it holds that $\tuple{M_1, M_2, \ldots, M_k}\models \f$ iff
$M_1\models \quant_1\pi_1,A_2$. 
If $\quant_1 = \forall$, the latter holds iff $M_1\cap \overline{A_2}= \emptyset$.
It holds that $M_1\cap \overline{A_2}\neq \emptyset$ iff there exists a lasso trace $\tau$ in $L(M_1)$ such that $\tau\in L(A_2)$. 
If $\quant_1 = \exists$, then $M_1\models \quant_1\pi_1 A_2$ iff 
$M_1\cap A_2\neq \emptyset$, which holds iff there exists a lasso trace $\tau$ in $L(M_1)$ such that $\tau\in L(A_2)$, proving the claim. 

Let $1<i<k$. We now assume the induction hypothesis, that $\tuple{M_1, M_2, \ldots, M_k}\models \f$ iff $\tuple{C_1, \ldots, C_i, M_{i+1},\ldots M_k}\models \f$, and prove that $\tuple{M_1, M_2, \ldots, M_k}\models \f$ iff $\tuple{C_1, \ldots, C_{i+1}, M_{i+2},\ldots M_k}\models \f$.  

We have that $\tuple{M_1, \ldots, M_k}\models \f$ iff $\tuple{M_1, \ldots, M_i, M_{i+1}}\models \alpha_{i+1}, A_{i+2}$, iff (by the induction hypothesis) $\tuple{C_1, \ldots, C_i, M_{i+1}}\models \alpha_{i+1}, A_{i+2}$.

Therefore, we prove that $\tuple{C_1, \ldots, C_i, M_{i+1}}\models \alpha_{i+1}, A_{i+2}$ iff $\tuple{C_1, \ldots, C_i, C_{i+1}}\models \alpha_{i+1}, A_{i+2}$.

If $\quant_i = \forall$, then if $\tuple{C_1, \ldots, C_i, M_{i+1}}\models \alpha_{i+1},A_{i+2}$, since $L(C_{i+1})\subseteq L(M_{i+1})$, we have that $\tuple{C_1, \ldots, C_i, C_{i+1}}\models \alpha_{i+1},A_{i+2}$. 
Now, suppose now that $\tuple{C_1, \ldots, C_i, C_{i+1}}\models \alpha_{i+1},A_{i+2}$, and let $c_1,c_2,\ldots c_{i}$ be lassos in $C_1,C_2,\ldots C_i$, respectively, with which, for every lasso $c_{i+1}\in C_{i+1}$, it holds that $\tuple{c_1,c_2,\ldots c_{i+1}}$ is in $L(A_{i+1})$. Let $\tau\in L(M_{i+1})$.
If, towards contradiction, $\tuple{c_1,\ldots,c_i,\tau}$ is not in $L(A_{i+1})$, then it is in $\overline{L(A_{i+1})}$. Then, using the accepting run of $\overline{L(A_{i+1})}$ on the joint run of $c_1,\ldots,c_k,\tau$, we can extract a lasso $c_{i+1}\in L(C_{i+1})$ such that $\tuple{c_1,c_2,\ldots c_i,c_{i+1}}\in \overline{L(A_{i+1})}$, and therefore is not in $L(A_{i+1})$, a contradiction.
Therefore, $\tuple{C_1,C_2,\ldots C_{i+1}}\models \alpha_{i+1},A_{i+2}$. 

If $\quant_i = \exists$, then if $\tuple{C_1, \ldots, C_i, C_{i+1}}\models A_{i+1}$, since $L(C_{i+1})\subseteq L(M_{i+1})$, we have that $\tuple{C_1, \ldots, C_i, M_{i+1}}\models A_{i+1}$.
For the other direction, let $c_1,c_2,\ldots c_i$ be as in the previous case, such that there exists a path $\tau\in L(M_{i+1})$ for which $\tuple{c_1,c_2,\ldots c_i,\tau}\in L(A_{i+1})$. Then we can extract an lasso $c_{i+1}\in L(C_{i+1})$ such that $\tuple{c_1,c_2,\ldots c_i,c_{i+1}}\in L(A_{i+1})$, and therefore in this case too, $\tuple{C_1,C_2,\ldots C_{i+1}}\models A_{i+1}$.


\end{proof} 

==> texs/simulation.tex <==
Let $M_1 = \tuple{Q,Q_0,R_1, L_1}, M_2 = \tuple{P,P_0,R_2,L_2}$ be Kripke structures, where $|Q|=n$. 

We construct a formula $S$ that is evaluated to $true$ iff there exists a simulation from $M_1$ to a sub-model of $M_2$ with at most $k$ states.

That is, there exists a set $P' = \{p_1,\ldots p_k\}\subseteq P$ and a relation $S\subseteq Q\times P'$ such that: 
\begin{enumerate}
    \item For every $(q,p)\in S$ it holds that $L(q)=L(p)$,
    \item For every $(q,p)\in S$, for every $q'$ such that $R_1(q,q')$ there exists $p'$ such that $R_2(p,p')$ and $(q',p')\in S$.
    \item For every $q\in Q_0$ there exists $p\in P_0$ such that $(q,p)\in S$.
\end{enumerate}

The formula $S$ is based on the algorithm for finding a maximal simulation from $M_1$ to $M_2$: First, construct 
$$S_0 = \{(q,p)|q\in Q, p\in P, L_1(q)=L_2(p)\}$$ 
Thus, $S_0$ is the set of all equally labeled pairs of states. Then, for $i\geq 1$, iteratively construct relations as follows, until reaching a fixed point $S$.  
$$S_i = \{(s,t)| (s,t)\in S_{i-1} \wedge \forall s':R_1(s,s')\exists t'(R_2(t,t') \wedge S_{i-1}(s',t'))\}$$

Notice that a fixed point $S_j$ is reached until at most $|Q|\cdot|P|$ iterations.

$M_2$ simulates $M_1$ iff for every $q\in Q_0$ there exists $p\in P_0$ such that $(q,p)\in S_j$. 

We encode this procedure by using the following formulas. 

\begin{equation}
\begin{aligned}
S \equiv \exists y_1\exists y_2 \dots\exists y_k \forall x (Q_0(x) \rightarrow \bigvee_{i=1}^{i=k} P_0(y_i)\wedge S_{k\cdot n}(x,y_i) ) 
\end{aligned}
\end{equation} 

The variables $y_1,\ldots y_k$ represent $k$ states in $M_2$. The formula $S$ requires that every state in $Q_0$ has a matching state in $P_0$ of the $k$ states, with which is satisfies $S_{k\cdot n}$, which represents the fixed point. 
The formulas $S_i$ are defined as follows. 

\begin{equation}
\begin{aligned}
 S_0(x,y)\equiv L_1(x)=L_2(y) 
\end{aligned}
\end{equation} 

\begin{equation}
\begin{aligned} S_{i}(x,y) \equiv & S_{i-1}(x,y)\wedge \forall x'( R_1(x,x') \rightarrow \exists y' (R_2(y,y') \\ & \wedge \bigvee_{i=1}^{i=k} (y_i=y') \wedge S_{i-1}(x',y'))
\end{aligned}
\end{equation}

Thus, $S_i$ exactly represents the iterative step, while requiring that the states of $M_2$ are only of the $k$ states of $S$. However, since $S_i$ contains two copies of $S_{i-1}$, this results in an exponential formula. 
Therefore, we construct an alternative formula which only uses a single copy of $S_{i-1}$, as follows. 

\begin{equation}
\begin{aligned}
    S_{i-1} = & \forall x' (R_1(x,x')\rightarrow \exists y' (R_2(y,y')\wedge \bigvee_{i=1}^{i=k} (y_i=y')\wedge \\
    & (\forall u\forall v( (u=x\wedge v=y)\vee (u=x'\wedge v=y')\rightarrow (S_{i-1}(u,v) ))))
    \end{aligned}
\end{equation} 


\subsection{A SAT encoding}

As another approach, we can encode such a simulation via a SAT formula, as follows. 
We assume a formula $q_i$ for every $q_i\in Q$, and we allocate a set $\{x_i\}_{i=1}^n$ for these formulas. 
For every $1\leq i\leq n$, we allocate a set of  variables $\{y_i^j\}_{j=1}^k$, which, intuitively, represent the set of states that are matched with $q_i$ in the simulation (if there are less than $k$ variables that are matched with $q_i$, then some of these variables will be assigned the same value in a satisfying assignment).
We also allocate a set of variables $\{y_i\}_{i=1}^k$. 
We define the following formulas.

\begin{enumerate}
    \item Every $x_i$ is a state in $M_1$ and every $y_i$ is a state in $M_2$: 
    $$\alpha_1 = \bigwedge_{i=1}^{n}Q(x_i)\wedge\bigwedge_{i=1}^{k} P(y_i)$$. 
    \item All the states in $M_2$ in the simulation are one of the $k$ $y$-states: 
    $$\alpha_2  = \bigwedge_{i=1}^{n}\bigwedge_{j=1}^{k} \bigvee_{t=1}^{k} y_i^j = y_t $$  
    \item All the states that are matched in the simulation are equally labeled: 
    $$\alpha_3 = \bigwedge_{i=1}^n\bigwedge_{j=1}^k L_1(x_i) = L_2(y_i^j)$$
    \item
    For every $(x,y)$ in the simulation,
    every successor state of $x$ has a matching successor state of $y$.
    $$\alpha_4 = \bigwedge_{i=1}^n\bigwedge_{j=1}^n R_1(x_i,x_j) \rightarrow \bigwedge_{t=1}^k\bigvee_{r=1}^k R_2(y_i^t,y_j^r)$$
    
\end{enumerate}

The formula $\alpha = \bigwedge_{i=1}^4\alpha_i$ is then satisfiable iff there exists a desired simulation. 
